The staircase property: How hierarchical structure can guide deep learning

This paper identifies a structural property of data distributions that enables deep neural networks to learn hierarchically. We define the "staircase" property for functions over the Boolean hypercube, which posits that high-order Fourier coefficients are reachable from lower-order Fourier coefficients along increasing chains. We prove that functions satisfying this property can be learned in polynomial time using layerwise stochastic coordinate descent on regular neural networks -- a class of network architectures and initializations that have homogeneity properties. Our analysis shows that for such staircase functions and neural networks, the gradient-based algorithm learns high-level features by greedily combining lower-level features along the depth of the network. We further back our theoretical results with experiments showing that staircase functions are also learnable by more standard ResNet architectures with stochastic gradient descent. Both the theoretical and experimental results support the fact that staircase properties have a role to play in understanding the capabilities of gradient-based learning on regular networks, in contrast to general polynomial-size networks that can emulate any SQ or PAC algorithms as recently shown.

==> auxiliarylemmas.tex <==

\section{Update lemmas}

\subsection{Upper bound on gradients if fewer than two active inputs}


\subsection{Characterization of stationary points of loss landscape for training an individual neuron}

\eb{figure out later how to best express the $M_1, M_2, M_3, \hat{f}(\emptyset)$ parameters. I lean towards adding them in later}

Consider the idealized loss function 
$$\ellt(a,b,c) = \frac{1}{2}(2ab - M_3)^2 + \frac{1}{2}(a^2 + b^2 + c + \hat{f}(\emptyset))^2$$

This is a cartoon version of the more complicated loss function that arises when you train a neuron with two inputs
$$g_1(x) = M_1 (x_{S_1} + h_1(x))$$ and $$g_2(x) = M_2 x_{S_2},$$ and the neuron is parametrized by $a,b,c$ and computes
$$g(x) = (a g_1(x) + b g_2(x))^2 + c.$$
We suppose that $|h_1(x)| \leq \delta_1$ for all $x$\eb{, and $\hat{h}_1(\{S_1\}) = 0$}. And we wish to train the parameters $w = (a,b,c)$ of this neuron so as to minimize the loss
\begin{align*}
\ell(w) &= \ell(a,b,c) \\
&= \frac{1}{2}\EE_x[(f(x) - g(x))^2],
\end{align*}
where $|f(x)| \leq M_4$ for all $x$ and $\hat{f}(S_1 \Delta S_2) = M_3$ and $\hat{f}(\emptyset) \leq \delta_0$.
\footnote{This in turn is still a cartoon, but we will see how to make the picture go to full generality soon.} We will analyze the loss $\ell$ by first proving that its gradients (suitably renormalized) are close to the gradients of $\ellt$.
Let us write the loss at $\ell(a / M_1, b / M_2, c)$:
\begin{align*}
\ell(a/M_1,b/M_2,c) \\
&= \frac{1}{2}\EE_x[((a g_1(x) / M_1 + b g_2(x) / M_2)^2 + c - f(x))^2] \\
&= \frac{1}{2}\EE_x[((a x_{S_1} + b x_{S_2})^2 + c - f(x) + ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2}))^2], & \mbox{expanding $g_1$ and $g_2$} \\
&= \frac{1}{2}\EE_x[\Delta(a,b,c,x)^2],
\end{align*}
where
\begin{align*}
\Delta(a,b,c,x) &= \Deltat(a,b,c,x) + ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2}) \\
\Deltat(a,b,c,x) &= (a x_{S_1} + b x_{S_2})^2 + c - f(x)
\end{align*}

\subsection{Comparing $\ell$ and $\ellt$: true loss versus idealized loss}
Now note that for any $a,b,c,x$ we have
\begin{align*}
|\Delta(a/M_1,b/M_2,c,x)| &= |(a x_{S_1} + b x_{S_2})^2 + c - f(x) + ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2})| \\
&\leq |(a x_{S_1} + b x_{S_2})^2 + c| + |f(x)| + |ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2})| \\
&\leq (|a|+|b|)^2 + |c| + M + |a| \delta_1 (|a| \delta_1 + 2|a| + 2|b|) \\
&:= U_1 \lesssim M + |a|^2 + |b|^2 + |c|
\end{align*}
And
\begin{align*}
|\Deltat(a,b,c,x)| &\leq (|a|+|b|)^2 + |c| + M := U_4 \lesssim M + |a|^2 + |b|^2 + |c|
\end{align*}
Let us compare $\Delta$ to $\Deltat$. For any $a,b,c,x$,
\begin{align*}
|\Delta(a/M_1,b/M_2,c,x) - \Deltat(a,b,c,x)| &= |ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2})| \\
&\leq |a| \delta_1 ||a|\delta_1 + 2|a| + 2|b|| \\
&:= U_2 \lesssim \delta_1 (|a|^2 + |ab|)
\end{align*}
Furthermore, for any $a,b,c,x$, let us compare the gradients of $\Deltat$ and $\Delta$:
\begin{align*}
&\|\nabla_{a,b,c} \Deltat(a,b,c,x) - \nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x)\| = \|\nabla_{a,b,c} (ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2})) \| \\
&= \sqrt{|\pd{}{a} (ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2})) |^2 + |\pd{}{b} (ah_1(x)(a h_1(x) + 2a x_{S_1} + 2b x_{S_2}))|^2} \\
&= \sqrt{|2h_1(x) (a h_1(x) + 2a x_{S_1} + b  x_{S_2})|^2 + |2h_1(x)(a x_{S_2})|^2} \\
&\leq \sqrt{|2\delta_1 (|a| \delta + 2|a| + |b|)|^2 + |2\delta_1 |a||^2} \\
&:= U_3 \lesssim \delta_1 (|a| + |b|)
\end{align*}
Finally, let us upper bound the gradient of $\Delta$:
\begin{align*}
\|\nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x)\| &\leq \|\nabla_{a,b,c} \Deltat(a,b,c,x)\| + \|\nabla_{a,b,c} ( \Delta(a/M_1,b/M_2,c,x) - \Deltat(a,b,c,x))\| \\
&\leq \|\nabla_{a,b,c} \Deltat(a,b,c,x)\| + U_3 \\
&= \|\nabla_{a,b,c} (a x_{S_1} + b x_{S_2})^2 + c - f(x)\| + U_3 \\
&= \sqrt{|2a + 2b x_{S_1} x_{S_2}|^2 + |2a x_{S_1} x_{S_2} + 2b|^2 + ||1|^2} + U_3 \\
&\leq \sqrt{|2a + 2b|^2 + |2a + 2b|^2 + ||1|^2} + U_3 \\
&:= U_5 \lesssim |a| + |b| + 1
\end{align*}
Using the above bounds, we may prove that the gradient of the true loss is close to the gradient of the idealized loss:
\begin{align*}
\|\nabla_{a,b,c} \ell(a/M_1,b/M_2,c) - \nabla_{a,b,c} \ellt(a,b,c)\| &= \|\EE_x[\Delta(a/M_1,b/M_2,c,x) (\nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x)) - \Deltat(a,b,c,x) (\nabla_{a,b,c} \Deltat(a,b,c,x))]\| \\
&\leq \EE_x[\|\Delta(a/M_1,b/M_2,c,x) (\nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x)) - \Deltat(a,b,c,x) (\nabla_{a,b,c} \Deltat(a,b,c,x))\|] \\
&\leq \EE_x[\|(\Delta(a/M_1,b/M_2,c,x) - \Deltat(a,b,c,x)) (\nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x))\| + \|\Deltat(a,b,c,x) (\nabla_{a,b,c} \Delta(a/M_1,b/M_2,c,x) - \nabla_{a,b,c} \Deltat(a,b,c,x))\|] \\
&\leq U_2 U_5 + U_4 U_3 \\
&:= U_6 \\
&\lesssim (\delta_1 (|a|^2 + |ab|))(|a| + |b| + 1) + (M + |a|^2 + |b|^2 + |c|)(\delta_1 (|a| + |b|)) \\
&\lesssim \delta_1 (M + |a|^2 + |b|^2 + |c|)(|a| + |b| + 1)
\end{align*}

\subsection{Approximate stationary points of idealized loss}

\eb{Assume $M_1, M_2 = 1$ in this section.}

For the analysis, we will actually study the $L^2$-regularized loss, where the weights between neurons (but not the biases) are regularized. Furthermore, during training, we will penalize high weights from internal layers more than weights from inputs, by having an amount $\lambda_1 \gg \lambda_2$ of $L^2$ regularization on weights from internal layers versus on weights from input neurons. The idealized regularized loss is:
\begin{align*}
\elltr(a,b,c) &= \ellt(a,b,c) + \frac{1}{2}(\lambda_1 a^2 + \lambda_2 b^2).
\end{align*}
And the true regularized loss is
\begin{align*}
\ellr(a,b,c) &= \ell(a,b,c) + \frac{1}{2}(\lambda_1 a^2 + \lambda_2 b^2)
\end{align*}
We now reason about what $a,b,c$ must be if $\|\nabla_{a,b,c} \ell(a,b,c)\|$ is small.

Suppose that $\|\nabla_{a,b,c} \ellr(a,b,c)\| \leq \epsilon'$. By the previous subsection, this implies $\|\nabla_{a,b,c} \elltr(a,b,c)\| \leq \epsilon := \epsilon' + U_6$.
We consider what we can say about $a,b,c$ if $\|\nabla_{a,b,c} \elltr(a,b,c)\| \leq \epsilon$. For clarity, we repeat the full definition of $\elltr$. Let $M_3 = \hat{f}(S_1 \Delta S_2)$:
$$\elltr(a,b,c) = \frac{1}{2}(2ab - M_3)^2 + \frac{1}{2}(a^2 + b^2 + c - \hat{f}(\emptyset))^2 + \frac{\lambda_1}{2} a^2 + \frac{\lambda_2}{2} b^2.$$

Hence,
\begin{align*}
\|\nabla \elltr \|^2 \geq |\pd{\elltr}{c}|^2 = (a^2 + b^2 + c - \hat{f}(\emptyset))^2
\end{align*}
So if $\|\nabla \elltr\| \leq \epsilon$ then $|a^2 + b^2 + c - \hat{f}(\emptyset)| \leq \epsilon$.

Further, let $\eta = (2ab - M_3)$. If $\|\nabla \elltr\| \leq \epsilon$ then 
$|2\eta b + (a^2 + b^2 + c - \hat{f}(\emptyset))(2a) + \lambda_1 a| \leq \epsilon$,
so
\begin{align*}
|2 \eta b + \lambda_1 a| \leq \epsilon(1+|a|),
\end{align*} and similarly
\begin{align*}
|2 \eta a + \lambda_2 b| \leq \epsilon(1+|b|).
\end{align*}

So $|a + 2 \eta b / \lambda_1| \leq \epsilon(1 + |a|) / \lambda_1$, which means
\begin{align*}
|2 \eta (-2\eta b / \lambda_1) + \lambda_2 b| \leq \epsilon(1+|b|) + 2 |\eta| \epsilon(1+|a|) / \lambda_1.
\end{align*}
So
\begin{align*}
|(-4 \eta^2 / \lambda_1) b + \lambda_2 b| \leq \epsilon ((1+|b|) + 2 |\eta| (1+|a|) / \lambda_1).
\end{align*}
So
\begin{align*}
|\lambda_2 - 4 \eta^2 / \lambda_1| |b| \leq \epsilon ((1+|b|) + 2 |\eta| (1+|a|) / \lambda_1).
\end{align*}
So
\begin{align*}
|\lambda_1 \lambda_2 - 4 \eta^2| |b| \leq \epsilon (\lambda_1 (1+|b|) + 2 |\eta| (1+|a|)).
\end{align*}
By a symmetric argument, flipping $a$ and $b$, we get
\begin{align*}
|\lambda_1 \lambda_2 - 4 \eta^2| |a|
&\leq \epsilon(\lambda_2 (1+|a|) + 2|\eta|(1+|b|))
\end{align*}

\textit{Case 1}: If $|\lambda_1 \lambda_2 - 4 \eta^2| \geq |M_3|/10$, then
$$\max(|a|,|b|) \leq 10 \epsilon (\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / \min(1,|M_3|).$$

\textit{Case 2}: If $|\lambda_1 \lambda_2 - 4 \eta^2| < |M_3|/10$, then it must be that $|\eta| < |M_3|/6$ (since \eb{$\lambda_1 \lambda_2 < |M_3| / 100$}). So $|2ab - M_3| < |M_3|/6$, which implies that $2ab \in [5M_3/6, 7M_3/6]$, and so $\max(|a|, |b|) \geq \sqrt{|M_3|}/4$.
In this case, it follows that
\begin{align*}
|\sqrt{\lambda_1 \lambda_2} - 2|\eta|| &= |\lambda_1 \lambda_2 - 4 \eta^2| / |\sqrt{\lambda_1\lambda_2} + 2|\eta|| \\
&\leq 2\epsilon(\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / (\sqrt{\lambda_1 \lambda_2} \max(|a|,|b|)) \\
& \leq 8\epsilon(\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / (\sqrt{\lambda_1\lambda_2|M_3|})
\end{align*}
Suppose that $\sgn(\lambda_1 a) = \sgn(2 \eta b)$, in which case we also have $\sgn(\lambda_2 b) = \sgn(2 \eta a)$.
Therefore, $|2 \eta b + \lambda_1 a| + |2 \eta a + \lambda_2 b| \geq \lambda_1 |a| + \lambda_2|b| > \min(\lambda_1,\lambda_2)(\max(|a|,|b|) \geq \min(\lambda_1,\lambda_2)(\sqrt{M_3}/8 + \max(|a|,|b|)/2) > \epsilon(1 + \max(|a|,|b|))$, since \eb{$\epsilon < \min(\lambda_1,\lambda_2) \sqrt{|M_3|} / 8$}. This is a contradiction. Hence, we must have

$\sgn(\lambda_1 a) \neq \sgn(2\eta b)$.
So $|\lambda_1 a| \leq |b \sqrt{\lambda_1 \lambda_2}| + (8\epsilon(\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / (\sqrt{\lambda_1\lambda_2|M_3|}))|b| + \epsilon(1+|a|).$

Thus, if $|a| = \max(|a|,|b|) \geq \sqrt{|M_3|}/4$, we have
$\sqrt{\lambda_1} \leq \sqrt{\lambda_2} + ((8\epsilon(\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / (\sqrt{\lambda_1\lambda_2|M_3|}))|b| + \epsilon(1+|a|)) / ((\sqrt{|M_3|}/4)\sqrt{\lambda_1})$. However this is a contradiction because the left-hand side is less than $\sqrt{\lambda_1}$, because \eb{$\epsilon$ is small enough and $\sqrt{\lambda_2} \ll \sqrt{\lambda_1}$}.

So it must be the case that $|b| = \max(|a|,|b|) \geq \sqrt{|M_3|}/4$. So
$|a/b| \leq \sqrt{\lambda_2/\lambda_1} + ((8\epsilon(\lambda_1 + \lambda_2 + 2|\eta|)(1+|a|+|b|) / (\sqrt{\lambda_1\lambda_2|M_3|}))|b| + \epsilon(1+|a|)) / ((\sqrt{|M_3|}/4)\lambda_1)$.

Hence we must have $|a/b| \leq 2\sqrt{\lambda_2/\lambda_1}$, since $\eps$ is small enough.


\paragraph{The conclusion of this subsection} is that if $\delta_1$ is a small enough polynomial, then the approximate stationary points of the true regularized loss correspond to either \textit{Case 1}, $|a|,|b|$ very small (decreasing linearly in $|\delta_1|$), or \textit{Case 2}, $2ab \approx M_3$ and $|a/b| \leq 2\sqrt{\lambda_2/\lambda_1}$.

\eb{Will also need to reason about $\ellr$, and not just about $\elltr$ -- to prove that the bias term is set appropriately after training the neuron.}

Combined with the reasoning about the stationary points, we will conclude that training a primed neuron either yields an approximately blank neuron, or it yields an approximate monomial with relative error at most $\delta_1(\sqrt{\lambda_2/\lambda_1} + 1) + 2\delta_0$.

Setting the ratio $\lambda_2 / \lambda_1$ small enough (smaller than $1/s$ that the error cannot compound substantially, we can get the simplest result.

If we initialize net to all zeros and then iteratively pick a neuron that we have not trained before [e.g., going layerwise], add a small polynomial-magnitude noise to its weights and train it only if the gradient is large enough, and round small weights down to zero, then we learn the hierarchical boolean function.

\eb{We also need to write smoothness of the network. And we need to write constant probability training argument. And the architecture needs to be shifted a tad.}

Eventually, with some more elaborate arguments, we will be able to get a more natural algorithm: initialize all weights to some small random value; in the outer loop you pick a steepest-descent neuron; in the inner loop you train it to stationarity (early stopping). You stop the outer loop once the steepest-descent neuron gradient is small (early stopping).




\subsection{Product of inputs is learned with constant probability}

\begin{lemma}[Small $a,b$ means high loss]
Suppose that $|a|,|b| \leq \epsilon'$, for some $\epsilon' < 1/\sqrt{2}$. Then we must have $\ell(a,b,c) \geq \frac{1}{2} - 2(\epsilon')^2$.
\end{lemma}
\begin{proof}
$\ell(a,b,c) \geq \frac{1}{2}(2ab - 1)^2 \geq \frac{1}{2}(2(\epsilon')^2 - 1)^2 \geq \frac{1}{2} - 2(\epsilon')^2$.
\end{proof}

\begin{lemma}[If signs are right at initialization, then we never go to a bad stationary point]
Suppose that we are training a primed neuron that has not been trained before, and that $\sgn(a_0b_0) = \sgn(1)$ and $c_0 = 0$ and $|a_0|,|b_0| \in [r_1,r_2]$ at initialization, where $0 < r_1 < r_2 \leq \sqrt{1}{2}$. Then if $r_2^4 \leq r_1^2 / 100$ and $r_2^2 (\lambda_1 + \lambda_2) \leq r_1^2 / 100$, and $r_1^2 > 2\epsilon^{(4)}$ at no point during training do we ever have $|a_t|,|b_t| \leq r_1 / 100$.
\end{lemma}
\begin{proof}
We note that $\ellr$ does not increase during training, so we must always have $\elltr(a_t,b_t,c_t) \leq \ellr(a_0,b_0,c_0) + \epsilon^{(4)} \leq \elltr(a_0,b_0,c_0) + 2\epsilon^{(4)}$\eb{controls difference between $\ellr$ and $\elltr$}. So by appealing to the previous lemma it suffices to show that $\elltr(a_0,b_0,c_0) < \frac{1}{2} - 2(\epsilon')^2 - 2\epsilon^{(4)}$. This is true because 
\begin{align*}
\elltr(a_0,b_0,c_0) &= \elltr(a_0,b_0,0) = \frac{1}{2}(2a_0b_0 - 1)^2 + \frac{1}{2}(a_0^2 + b_0^2 + 0)^2 + \frac{1}{2}(\lambda_1 a_0^2 + \lambda_2 b_0^2) \\
&\leq \frac{1}{2}(2r_1^2 - 1)^2 + \frac{1}{2}(2r_2^2)^2 + \frac{1}{2}(\lambda_1 r_2^2 + \lambda_2 r_2^2) \\
&\leq \frac{1}{2} - 2r_1^2 + (2r_1^4 + 2r_2^4 + \frac{1}{2}(\lambda_1 r_2^2 + \lambda_2 r_2^2) \\
&\leq \frac{1}{2} - 2r_1^2 + r_2^2 (4r_2^2 + (\lambda_1 / 2 + \lambda_2 / 2)) \\
&\leq \frac{1}{2} - r_1^2 + r_2^2 (4r_2^2 + (\lambda_1 / 2 + \lambda_2 / 2)) - 2\epsilon^{(4)} \\
&\leq \frac{1}{2} - 95 r_1^2 / 100  - 2 \epsilon^{(4)} \\
&\leq \frac{1}{2} - 2(r_1 / 100)^2 - 2\epsilon^{(4)}
\end{align*}
\end{proof}
We conclude that if a primed neuron is trained then with constant probability (the probability that $\sgn(ab) = \sgn(1)$ and that $a,b$ are in the correct range) the correct stationary point is reached after training.

\subsection{Upper bound on magnitude of untrained neuron}

\subsection{Lower bound on magnitude of trained neuron}

\subsection{Lower bound on gradient for primed neuron}

\begin{lemma}

\end{lemma}

\subsection{Upper bound on gradient for neuron with no active inputs}

\subsection{Upper bound on gradient for neuron with one active input}

\subsection{Upper bound on gradient for untrained neuron with one two active inputs}

\subsection{Upper bound on gradient for trained neuron}

\subsection{The freshness of the randomness in selection of how to combine two active neurons}

It should only depend on the weights coming from them -- all other terms, which we cannot control, should be lower-order corrections.

The goal of this is to prove that the structural invariant that every neuron has at most 3 input edges from active neurons is maintained.

\subsection{Analyzing the stationary points of the idealized loss, when we add inputs from untrained neurons}

\subsection{Analyzing the stationary points of the idealized loss, when we add small-weight outputs to untrained neurons}

\section{Local update result}

{\color{gray}
\eb{All $O()$ and $\Omega()$ notation will be replaced by constants.}\eb{proofs are rough and will be polished, but just want to get it all down first}



In this section, we show the main lemma that proves that gradient descent on a neuron's parameters can learn the product of the inputs. In this simple setting, let $M_1,M_2,M_3 \in \RR$ be numbers. We have access to two inputs computing functions $f_1(x) = M_1 x_1$ and $f_2(x) = M_2 x_2$, weighted by $a$ and $b$ respectively and it returns the function $(a x_1 + b x_2)^2 + c$. Suppose we train the neuron to learn the function $M_3 x_1x_2$. 
For technical reasons, we also add regularization on $a$ and $b$ of polynomial magnitude (with no regularization on the bias term $c$\footnote{$c$ is naturally regularized in some sense, by the fact that $a$ and $b$ are regularized.}. This results in the following loss:
\begin{definition}[Simple loss function]
Let $0 < \lambda_1, \lambda_2 < 1$ be $L^2$ regularization parameters. The loss is $\ell(a,b,c) = \frac{1}{2}(2ab M_1 M_2 - M_3)^2 + \frac{1}{2}(a^2 M_1^2 + b^2 + M_2^2 + c)^2 + \frac{\lambda_1}{2} a^2 + \frac{\lambda_2}{2} b^2$.
\end{definition}
This is a nonconvex objective, so it is nontrivial to train. The main lemma in this section proves that polynomially-many steps of noisy gradient descent with an appropriate, random initialization will reach an approximate global optimum.

\subsection{Proof of GD convergence}



\eb{Insert GD for ERM -- empirical loss vs. true loss, empirical gradients vs. true gradients}
\begin{lemma}[Empirical loss is well behaved]\label{lem:empappx}
With high probability, the empirical loss $\ellh$ satisfies the following properties for any $\|w\| \leq R$, \eb{specify $\eps$, $R$, $L$}
\begin{enumerate}
\item Approximates the true loss: $|\ellh(w) - \ell(w)| \leq \eps$.
\item Gradients approximate the true gradients: $\|\nabla \ellh(w) - \nabla \ell(w)\| \leq \eps$.
\item Smooth $\|\nabla^2 \ellh(w)\| \leq L$.
\end{enumerate}
\end{lemma}

\begin{theorem}[Local update theorem on empirical loss landscape]
Let $\alpha, \lambda_1, \lambda_2, \eps > 0$, and train $\nabla \ellh$ with gradient descent of step size $\alpha \ll O(1/\lambda_1 + 1/\lambda_2)$ starting from $w_0 = (a_0,b_0,c_0) \approx 0$. I.e., for all $t \geq 0$
$$w_{t+1} = w_t - \alpha \nabla \ellh(w_t).$$
Then for $t \geq \dots$, we have
$$ $$
\end{theorem}

The proof of the local update theorem is based on several auxiliary lemmas. The first is that the loss is always non-increasing, which follows due to smoothness of the objective in a ball and the $L^2$ regularization that means that the parameters never exit the ball.
\begin{lemma}[Non-increasing loss]
The loss is always non-increasing, and $a_t,b_t \leq \dots $ and $c \leq \dots $ throughout. \eb{condition on $M_1,M_2,M_3$}
\end{lemma}
\begin{proof}
\end{proof}

Since we choose $a_0,b_0,c_0$ to be close to zero at initialization, we can bound the loss at initialization. 
\begin{lemma}[Bound on loss at initialization]
If $|a_0|,|b_0|,|c_0| \leq$, then $\ellh(a_0,b_0,c_0) \leq $
\end{lemma}

We now analyze the trajectory of gradient descent around initialization. We split the analysis into the cases that $\sgn(a_0 b_0 M_1 M_2) \neq \sgn(M_3)$ and $\sgn(a_0 b_0 M_1 M_2) = \sgn(M_3)$.

\subsection{Case that $\sgn(a_0 b_0 M_1 M_2) \neq \sgn(M_3)$ at initialization}
In this subsection we analyze the case in which $\sgn(a_0 b_0 M_1 M_2) \neq \sgn(M_3)$ at initialization. The analysis shows that after a small, polynomial number of iterations of gradient descent we quickly reach the regime in which $\sgn(a_t b_t M_1 M_2) = \sgn(M_3)$. The intuition behind the result of this subsection is that the neuron being trained approximately computes $a_t b_t M_1 M_2 x_{S_1} x_{S_2}$ up to an additive constant. Thus, in order to match the $M_3 x_{S_1} x_{S_2}$ monomial in the target function, $a_t$ and $b_t$ evolve so that the sign of $a_t b_t M_1 M_2$ matches the sign of $M_3$.

In the formal analysis, care must be taken to lower-bound the rate of change of the loss. In particular, we must avoid the saddle point in the loss landscape that occurs at $a,b = 0$, and also we must avoid the vanishingly small gradients that would slow down the rate of loss decrease if $a,b$ were to become too close (e.g., exponentially close) to zero. For this, we must use two properties of the random initialization: (1) that with high probability $|a_0|$, $|b_0|$, and $|c_0|$ are of polynomially-small magnitude (2) that with high probability the ratio $||a_0| - |b_0||$ is bounded away from 1. These two conditions appear as deterministic conditions in the following lemma, although they can be shown to hold with high probability at our random initialization, as we will show when we apply the lemma to prove Theorem~\ref{thm:noisylocalupdate}:
\begin{lemma}[Flipping the sign: case $\lambda_1 = \lambda_2$] \label{lem:sameregbadsign}
Suppose that the regularization parameters for the two neuron inputs are equal: i.e., $\lambda = \lambda_1 = \lambda_2$. If $\sgn(a_0 b_0 M_1 M_2) \neq \sgn(M_3)$ and $||a_0| - |b_0|| \geq \eb{do}$ and $\ell(a_0,b_0,c_0) \leq \eb{do}$, then there is a timestep $t \leq \eb{do}$ such that
$$\sgn(a_t b_t M_1 M_2) = \sgn(M_3)$$ and $$\max(|a_t|,|b_t|) \geq \eb{do}$$ and $$\ell(a_t,b_t,c_t) \leq \eb{do}$$
\end{lemma}

\begin{claim}\label{claim:signflipbiastermbound}
Suppose $\sgn(a_0b_0 M_1 M_2) \neq \sgn(M_3)$ and $\sgn(a_1) = \sgn(a_0)$ and $\sgn(b_1) = \sgn(b_0)$. Then
$|a_{t+1}| - |b_{t+1}| = $
\end{claim}

\begin{proof}
Suppose $T$ is an integer such that $\sgn(a_{t+1}) = \sgn(a_{t})$ and $\sgn(b_{t+1}) = \sgn(b_{t})$ for all $t \in \{0,\ldots,T-1\}$. Then by induction on $t$ we must have \begin{equation}\label{eq:flipsignsignnotflipped}\sgn(a_{t} b_{t} M_1 M_2) \neq \sgn(M_3)\end{equation} for all $t \in \{0,\ldots,T\}$. In particular, since the loss does not decrease and $\ell(w_t) \leq \ell(w_0) \leq M_3^2 + M_3^2 / 4$,  Claim~\ref{claim:signflipbiastermbound} implies
\begin{equation}\label{eq:flipsignrelativelyunbiased}|a_t^2 + b_t^2 + c_t| \leq M_3 / 4 \mbox{ for all } t \in \{0,\ldots,T\}.\end{equation}
Let us now write the gradient descent update equation for $a_{t+1}$. For ease of notation, define \begin{align*}\kappa_t &= 2a_tb_t M_1 M_2 - M_3, \mbox{ and } \\ \eta_t &= a_t^2 M_1^2 + b_t^2 M_2^2 + c_t\end{align*}
Using these to express the update equation for $a_{t+1}$, we write:
\begin{align*}
a_{t+1} &= a_{t} - \alpha\pd{\ellh(w_{t})}{a} \\
&= a_t - \alpha(\kappa_t (2b_t M_1M_2) + \lambda a_t + \eta_t (2a_{t} M_1^2)) - \alpha\left(\pd{\ellh(w_t)}{a} - \pd{\ell(w_t)}{a}\right)
\end{align*}
If $t \in \{0,\ldots,T-1\}$, then it follows from \eqref{eq:flipsignsignnotflipped} that $\kappa_t \leq - M_3$. Furthermore, it follows from \eqref{eq:flipsignrelativelyunbiased} that $|\eta_t| \leq M_3 / 4$. Finally, 
\begin{align*}
    |a_{t+1}| &= (1 - \alpha \lambda) \cdot |a_t| - \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)| \cdot |b_t| + \xi_{t+1}
\end{align*}


where $\xi_{t+1}$ and $\psi_{t+1}$ are error terms that can be bounded by the triangle inequality:
\begin{align*}|\xi_{t+1}| &\leq \alpha|(a_t^2 M_1^2 + b_t^2 M_2^2 + c_t)(2a_t M_1^2)| + \alpha|\pd{\ellh(w_t)}{a} - \pd{\ell(w_t)}{a}| \\
&\leq \alpha |\eb{do}| + \alpha \epsilon, & \mbox{using $\|\nabla \ellh(w_t) - \nabla \ell(w_t)\| \leq \epsilon$  from Lemma~\ref{lem:empappx}} \\
&\leq \alpha |\eb{do}| + \alpha \epsilon, & \mbox{using the above claim}
\end{align*}

A similar calculation for $b_t$ shows that:
\begin{align*}
b_{t+1} &= b_t - \alpha(\pd{\ellh(w_t)}{b}) \\
&= b_t - \alpha((a_t^2 M_1^2 + b_t^2 M_2^2 + c_t)(2b_t M_2^2) + (2a_tb_tM_1M_2 - M_3)(2a_tM_1M_2) + \lambda b_t) - \alpha(\pd{\ellh(w_t)}{b} - \pd{\ell(w_t)}{b})
\end{align*}

\begin{align*}
|a_{t+1}| &= (1 - \alpha \lambda) \cdot |a_t| - \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)| \cdot |b_t| + \xi_{t+1} \\
|b_{t+1}| &= (1 - \alpha \lambda) \cdot |b_t| - \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)| \cdot |a_t| + \psi_{t+1},
\end{align*}
Similarly,
\begin{align*}
|\psi_{t+1}| &\leq \alpha |\eb{do}| + \alpha \epsilon.
\end{align*}

\begin{align*}
|a_{t+1}| - |b_{t+1}| &= |a_t - \alpha \pd{\ellh(w_t)}{a}| - |b_t - \alpha \pd{\ellh(w_t)}{b}|
\end{align*}
\end{proof}

In order to prove the lemma, let us first prove the following auxiliary claim:
\begin{claim}
If $\sgn(a b M_1 M_2) \neq \sgn(M_3)$ and $\ell(a,b,c) \leq M_3^2 + \eb{do}$, then $(a^2 M_1^2 + b^2 M_2^2 + c)^2 \leq \eb{do}$

The above claim is useful in the following way: since $\ell(w_t) \leq \ellh(w_t) + \epsilon \leq \ellh(w_0) + \epsilon \leq \ell(w_0) + 2\epsilon$ throughout training, we may guarantee the following: if $\sgn(a_tb_tM_1M_2) \neq \sgn(M_3)$ then $|a_t^2 M_1^2 + b_t^2 M_2^2 + c_t| \leq \eb{do}$. 
\end{claim}
\begin{proof}
From the first assumption, we know $(2ab M_1 M_2 - M_3)^2 \geq M_3^2$. Thus,
$\frac{1}{2}(a^2 M_1^2 + b^2 M_2^2 + c)^2 \leq \ell(a,b,c) - \left(\frac{\lambda_1 a^2}{2} - \frac{\lambda_2 b^2}{2} +  \frac{1}{2}(2a b M_1 M_2 - M_3)^2\right) \leq \ell(a,b,c) - M_3^2 \leq \eb{do}$.
\end{proof}
We may prove Lemma~\ref{lem:sameregbadsign}
\begin{proof}
Writing out the update equations for gradient descent, we have:
\begin{align*}
a_{t+1} &= a_t - \alpha(\pd{\ellh(w_t)}{a}) \\
&= a_t - \alpha((a_t^2 M_1^2 + b_t^2 M_2^2 + c_t)(2a_t M_1^2) + (2a_tb_tM_1M_2 - M_3)(2b_tM_1M_2) + \lambda a_t) - \alpha(\pd{\ellh(w_t)}{a} - \pd{\ell(w_t)}{a})
\end{align*}
\begin{align*}
b_{t+1} &= b_t - \alpha(\pd{\ellh(w_t)}{b}) \\
&= b_t - \alpha((a_t^2 M_1^2 + b_t^2 M_2^2 + c_t)(2b_t M_2^2) + (2a_tb_tM_1M_2 - M_3)(2a_tM_1M_2) + \lambda b_t) - \alpha(\pd{\ellh(w_t)}{b} - \pd{\ell(w_t)}{b})
\end{align*}
Suppose that $\sgn(a_{t+1}) = \sgn(a_t)$ and $\sgn(b_{t+1}) = \sgn(b_{t})$. Then
\begin{align*}
|a_{t+1}| &= (1 - \alpha \lambda) \cdot |a_t| - \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)| \cdot |b_t| + \xi_{t+1} \\
|b_{t+1}| &= (1 - \alpha \lambda) \cdot |b_t| - \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)| \cdot |a_t| + \psi_{t+1},
\end{align*}
where $\xi_{t+1}$ and $\psi_{t+1}$ are error terms that can be bounded by the triangle inequality:
\begin{align*}|\xi_{t+1}| &\leq \alpha|(a_t^2 M_1^2 + b_t^2 M_2^2 + c_t)(2a_t M_1^2)| + \alpha|\pd{\ellh(w_t)}{a} - \pd{\ell(w_t)}{a}| \\
&\leq \alpha |\eb{do}| + \alpha \epsilon, & \mbox{using $\|\nabla \ellh(w_t) - \nabla \ell(w_t)\| \leq \epsilon$  from Lemma~\ref{lem:empappx}} \\
&\leq \alpha |\eb{do}| + \alpha \epsilon, & \mbox{using the above claim}
\end{align*}
Similarly,
\begin{align*}
|\psi_{t+1}| &\leq \alpha |\eb{do}| + \alpha \epsilon.
\end{align*}

So if $\sgn(a_{t+1}) = \sgn(a_t)$ and $\sgn(b_{t+1}) = \sgn(b_{t})$ for all $t \in [T]$, the following recurrence holds:
\begin{align*}
|a_{t+1}| - |b_{t+1}| = (|a_t| - |b_t|)(1 - \alpha \lambda + \alpha|(2M_1M_2)(2a_tb_tM_1M_2 - M_3)|) + \xi_{t+1} - \psi_{t+1}
\end{align*}
Therefore, since $|M_1M_2M_3| \geq \lambda$, and also because we have maintained $\sgn(a_tb_tM_1M_2) \neq \sgn(M_3)$, we obtain
\begin{align*}
||a_{t+1}| - |b_{t+1}|| &\geq ||a_t| - |b_t||(1 + \alpha(|2M_1M_2 M_3| - \lambda)) - (|\xi_{t+1}| + |\psi_{t+1}|) \\
&\geq ||a_t| - |b_t||(1 + \alpha |M_1M_2M_3|) - (|\xi_{t+1}| + |\psi_{t+1}|) \\
\end{align*}

Thus, using the upper bounds on $|\xi_{t+1}|$ and $|\psi_{t+1}|$, 
However, this is a contradiction because it would imply that $a_{t+1}^2 + b_{t+1}^2 \geq \eb{do}$, which would mean that $\ell(a_{t+1},b_{t+1},c_{t+1}) \geq \frac{\lambda}{2}(a_{t+1}^2 + b_{t+1}^2) \gg \ell(a_0,b_0,c_0)$. 

Since we have derived a contradiction, there must be $t+1 \in [T]$ such that $\sgn(a_{t+1}) \neq \sgn(a_t)$ or $\sgn(b_{t+1}) \neq \sgn(b_t)$. Pick the first such $t$. From the recurrence relation until this point, we know that $||a_t| - |b_t|| \geq ||a_0| - |b_0||$, so $\max(|a_t|,|b_t|) \geq ||a_0| - |b_0|| / 2 \geq 1 / \poly(n) \gg THE ERROR IN THE GRADIENT$. Therefore, it must be the case that only one of the two coordinates $a_t,b_t$ changes sign. And also since the other one cannot decrease too fast on this iteration, this means that $\max(|a_{t+1}|,|b_{t+1}|)$ is lower-bounded by $1/\poly(n)$ and also that $\sgn(a_{t+1}b_{t+1}M_1M_2) = \sgn(M_3)$. \eb{formalize}








\end{proof}

We prove a similar lemma in the case that one of the regularization parameters is much larger than the other (for the SGD proof later):
\begin{lemma}[Flipping the sign: case $\lambda_1 \gg \lambda_2$]

\end{lemma}

Once the regime with $\sgn(a_t b_t M_1 M_2) = \sgn(M_3)$ has been reached, we may apply the analysis that we would apply as if we had merely initialized in that regime (i.e., the analysis in

\subsection{The trick that simplifies these analyses is}
to stop after a random number of iterations within a certain uniform range. The probability of being near zero activation or being near the final activation value is $1 - 1 / \poly(n)$.
This means that we can brush many of the nasty details of the analysis under the rug (once we add the truncation step, that is). We can avoid getting stuck in a saddle region, say.

\subsection{Case that $\sgn(a_0 b_0 M_1 M_2) = \sgn(M_3)$ at initialization}
\begin{lemma}
Suppose that $\sgn(a_0 b_0 M_1 M_2) = \sgn(M_3)$
\end{lemma}
 and also $\max(|a_t|,|b_t|)$ is polynomially lower-bounded, is reached. In this regime, we prove that the loss decreases quickly to at most $1/2$.
















\section{Coordinate descent}

In this section, we will prove that a simple neural network architecture, trained with a noiseless coordinate descent procedure that has access to the (noiseless) gradient of the loss, will learn hierarchical boolean functions.


\subsection{OLD: Noiseless regularized analysis (simple version of main local update lemma for neuron-wise updates)}


\eb{The proofs in this section have some missing parts right now.}

In this section, we show the main lemma that proves that gradient descent on a neuron's parameters can learn the product of the inputs. In this simple setting, the neuron has two inputs $x_1$ and $x_2$ and it returns the function $(a x_1 + b x_2)^2 + c$. For technical reasons, these proofs require regularization on $a$ and $b$ of polynomial magnitude to work. And there is no regularization on the bias term $c$ (which is naturally regularized in some sense because $a$ and $b$ are regularized). For simplicity, in this section we deal with trying to learn the function $x_1x_2$. This results in the following loss:
\begin{definition}[Simple loss function]
Let $0 < \lambda < 1$ be the $L^2$ regularization parameter. The loss is $\ell(a,b,c) = \frac{1}{2}(2ab - 1)^2 + \frac{1}{2}(a^2 + b^2 + c)^2 + \frac{\lambda}{2} (a^2 + b^2)$.
\end{definition}
This is a nonconvex objective, so it is nontrivial to train. The objective of this section is to prove that polynomially-many steps of gradient descent with an appropriate initialization will get us exponentially-close to a global optimum. These ideas will be extended in the next section to the more complicated case where the inputs to the neuron are noisy, and the function we are trying to learn has nonzero fourier coefficients apart from $\{1,2\}$.\eb{All $O()$ and $\Omega()$ notation will be replaced by constants.}\eb{proofs are rough and will be polished, but just want to get it all down first}

\paragraph{Gradient descent} Let $0 < \alpha < O(\lambda)$. Train the loss function $\ell(w) = \ell(a,b,c)$ with gradient descent of step size $\alpha$ starting from $w_0 = (a_0,b_0,c_0) \approx 0$. Then the main result of this section is:

\begin{theorem}[Simple local update theorem]
If we set $a_0,b_0,c_0 \sim \cN(0,1)$, then there is a constant $C$ such that for any $0 < \delta < 1/2$ and $T \geq (\log(1/\delta),1/\alpha,1/\lambda)^C$, we have the bound $$\ell(a_t,b_t,c_t) \leq \delta$$ with probability $\geq 1 - \delta$.
\end{theorem}
\begin{proof}
If $2a_0b_0 \geq \lambda$, then the bound $\ell(a_t,b_t,c_t) \leq \delta$ with probability one follows from the lemmas below. \eb{I have yet to write the other cases' proofs (i.e., $a_0,b_0$ are initialized to too small, and $\sgn(a_0) \neq \sgn(b_0)$). However, these other cases have simple proofs as well.}
\end{proof}



\begin{lemma}
The loss is always non-increasing, and $a_t,b_t \leq O(1/\sqrt{\lambda})$ and $c \leq 1/\lambda$ throughout.
\end{lemma}
\begin{proof}
We start out with a loss of $\approx 1$. We prove by induction that the loss always decreases. Since the loss is $O(1)$ on each step, we must have $a_t,b_t \leq O(1/\sqrt{\lambda})$ and hence $c_t \leq O(1/\lambda)$  always. If we look at second derivatives, we have $\frac{\partial^2 \ell}{\partial a^2} = \frac{\partial a(a^2 + b^2 + c)}{\partial a} + \lambda = (a^2 + b^2 + c) + 2a^2 + \lambda \leq 10 / \lambda$. Symmetrically, $\frac{\partial^2 \ell}{\partial b^2} \leq 10/ \lambda$. And $\frac{\partial^2 \ell}{\partial c^2} = 1 \leq 10 / \lambda$. And $\frac{\partial^2 \ell}{\partial a \partial b} = \frac{\partial a(a^2 + b^2 + c)}{\partial b} = 2ab$. And $\frac{\partial^2 \ell}{\partial a \partial c} = \frac{\partial (a^2 + b^2 + c)}{\partial a} = 2a \leq 10 / \lambda$. And $\frac{\partial^2 \ell}{\partial b \partial c} \leq 10 / \lambda$. As a consequence, $\|\nabla^2 \ell\| \leq O(1 / \lambda)$. So since $\alpha = O(1/\lambda)$ for appropriately small constant in the big-Oh notation, one step of gradient descent cannot decrease the loss.
\end{proof}








\subsection{Analysis for $a,b \geq 0$}
In this section, we will consider the dynamics in the region $a,b \geq 0$.

A simple computation yields
\begin{align*}\|\nabla \ell\|^2 &= \left(\pd{\ell}{a}\right)^2 + \left(\pd{\ell}{b}\right)^2 + \left(\pd{\ell}{c}\right)^2 \\
&= \left(\lambda a + (2ab - 1)(2b) + (a^2 + b^2 + c)(2a)\right)^2 + \left(\lambda b + (2ab - 1)(2a) + (a^2 + b^2 + c)(2b)\right)^2 + (a^2 + b^2 + c)^2.\end{align*}

The first result is that gradient descent remains in the region $\{a,b \geq 0\}$ region once it has entered.
\begin{lemma}
If $a_0,b_0 \geq 0$ and $a_0,b_0,c_0 \in [L,L]$ and $\alpha \leq O(1/(L^2 + \sqrt{\lambda}))$, then $a_t,b_t \geq 0$ for all $t \geq 0$.
\end{lemma}
\begin{proof}
$a_1 = a_0 - \alpha (\lambda a_0 + (2a_0b_0 - 1)(2b_0) + (a_0^2 + b_0^2 + c_0)(2a_0))$. If $2a_0b_0 - 1 \leq 0$, then $a_1 \geq a_0 - \alpha (\lambda + 2(a_0^2 + b_0^2 + c_0))(a_0) = a_0 ( 1 - \alpha (\lambda + 2(a_0^2 + b_0^2 + c_0))) \geq 0$, where the last inequality holds because both terms in the product are positive. On the other hand, if $2a_0 b_0 - 1 \geq 0$, then $a_1 \geq a_0 (1 - \alpha (\lambda + 2(a_0^2 + b_0^2 + c_0))) - b_0 (\alpha (2a_0b_0 - 1))$. In this case, since $2 a_0 b_0 \geq 1$, we must have $a_0 \geq 1/(2b_0) \leq 1/(2L)$. So $b_0 / a_0 \geq 1 / (2L^2)$. So $a_1 \geq a_0 (1 - \alpha(\lambda + 2(a_0^2 + b_0^2 + c_0))) - \alpha a_0 (2 b_0^2 - (b_0 / a_0)) \geq a_0 / 2 - \alpha a_0 L^2 \geq 0$.
\end{proof}

\paragraph{Progress bounds}
We also note the following lower-bounds on progress made in the region $\{a_t,b_t \geq 0\}$.

\begin{itemize}
\item If $|a^2 + b^2 +c| \geq \lambda/4$, then $\|\nabla \ell\|^2 \geq (a^2 + b^2 + c)^2 \geq \lambda^2 / 16$.

\item Otherwise, if $|a^2 + b^2 + c| \leq \lambda / 4$, then
\begin{itemize}
\item if $2ab \geq 1$, then since $\lambda/2 > 2|a^2 + b^2 + c|$, we have
\begin{align*}\|\nabla \ell\|^2 &\geq (\lambda a + (2ab - 1)(2b) - |a^2 + b^2 + c|(2a))^2 + (\lambda b (2ab - 1)(2a) - |a^2 + b^2 + c|(2b))^2 \\
&\geq (\lambda a / 2 + (2ab - 1)(2b))^2 + (\lambda b / 2 + (2ab - 1)(2a))^2 \\
&\geq (\lambda a / 2)^2 + (\lambda b / 2)^2 \\
&\geq (a^2 + b^2) \lambda^2 / 4 \\
&\geq (2ab) \lambda^2 / 4 \\
&\geq \lambda^2 / 4
\end{align*}
\item if $2ab \in [1 - \lambda / 8, 1 + \lambda / 8]$, then $3\lambda/4 > 2|2ab - 1| + 2|a^2 + b^2 + c|$, so
\begin{align*}
    \|\nabla \ell\|^2 &\geq \left(\lambda \max(a,b) + (2ab - 1)(2\min(a,b)) + (a^2 + b^2 + c)(2\max(a,b))\right)^2 \\
    &\geq (\lambda \max(a,b) / 4)^2 \\
    &\geq ((a^2 + b^2) / 2) \lambda^2 / 16 \\
    &\geq ((2ab) / 2) \lambda^2 / 16 \\
    &\geq \lambda^2 / 64, & \mbox{using $2ab \geq 1 - \lambda / 4 \geq 1/2$}.
\end{align*}

\item if $2ab \in [0, 1 - 4\lambda/5]$, then $2|2ab - 1| - (\lambda + 2|a^2 + b^2 + c|) \geq |2ab - 1| / 10$, so 
\begin{align*}
\|\nabla \ell\|^2 &\geq ((2ab - 1)(2 \max(a,b)) + (a^2 + b^2 + c)(2\min(a,b)) + \lambda (\min(a,b)))^2 \\
&\geq (|2ab - 1|(2\max(a,b)) - |a^2 + b^2 + c|(2 \min(a,b)) - \lambda (\min(a,b)))^2 \\
&\geq ((2ab - 1) \max(a,b) / 2)^2 \\
&\geq ((a^2 + b^2) / 2) (2ab - 1)^2 / 4 \\
&\geq ((2ab) / 2) (2ab - 1)^2 / 4 \\
&\geq (2ab) \lambda^2 / 8
\end{align*}

\item if $2ab \in [1 - \lambda, 1 - \lambda / 8]$ and $a^2 + b^2 \geq 32$, then $\max(a,b)^2 \geq 16$ so $\max(a,b) \geq 4$. Since $2ab \leq 1$ we also have $\min(a,b) \leq \frac{1}{8}$.
Therefore, since $\lambda \max(a,b) \geq \lambda(2\min(a,b)) + (\lambda / 4)(2\max(a,b)) + \lambda$
\begin{align*}
\|\nabla \ell\|^2 &\geq \left(\lambda \max(a,b) - |2ab - 1|(2\min(a,b)) + (a^2 + b^2 + c)(2\max(a,b))\right)^2 \\
&\geq \left(4\lambda - |2ab - 1|/4 + 8(a^2 + b^2 + c)\right)^2 \\
&\geq \lambda^2
\end{align*}
\end{itemize}
\end{itemize}

The regions of $\{a,b \geq 0\}$ that remain to be reasoned about are $\{2ab \in [1-4\lambda/5, 1 - \lambda / 8], |a^2 + b^2  + c| \leq \lambda / 4, a^2 + b^2 \leq 32\}$ and $\{2ab \in [0,\lambda], |a^2 + b^2 + c| \leq \lambda / 4\}$.

\begin{lemma}

\end{lemma}

\paragraph{Once loss is at most $1 - \lambda$, we reach a loss of at most $1/2$ pretty quickly}
\begin{lemma}\label{lem:lossleq1minuslambda}
If $\ell(a,b,c) \leq 1 - \lambda$ then $2ab \geq \lambda$.
\end{lemma}
\begin{proof}
Since $\ell(a,b,c) \geq (2ab - 1)^2$.
\end{proof}

\begin{lemma}
If $2ab \in [1-4\lambda/5,1 - \lambda/ 8], |a^2 + b^2 + c| \leq \lambda / 4, a^2 + b^2 \leq 32 $, then $\ell(a,b,c) \leq 1/2$.
\end{lemma}
\begin{proof}
\begin{align*}
\ell(a,b,c) &= \frac{\lambda}{2} (a^2 + b^2) + \frac{1}{2}(2ab-1)^2 + \frac{1}{2}(a^2 + b^2 + c)^2 \\
&\leq 16\lambda + \lambda^2 / 2 + (\lambda / 4)^2 / 2 \\
&\leq 17\lambda \\
&\leq 1/2.
\end{align*}
\end{proof}

\begin{lemma}
If $a_0,b_0,c_0$ is such that $\ell(a_0,b_0,c_0) \leq 1 - \lambda$, then $\ell(a_T,b_T,c_T) \leq 1/2$ for any $T \geq 128 / (\alpha \lambda^4)$.
\end{lemma}
\begin{proof}
Since the loss does not decrease, we have $\ell(a_t,b_t,c_t) \leq \ell(a_0,b_0,c_0) \leq 1 - \lambda$ for all $t \geq 0$. By Lemma~\ref{lem:lossleq1minuslambda}, therefore $2a_t b_t \geq \lambda$ for all $t \geq 0$. Assume by contradiction that $\ell(a_t,b_t,c_t) > 1/2$ for all $t \in \{0,\ldots,T\}$. In this case, by the previous lemma for any $t \in \{0,\ldots,T\}$ we must have $(a_t,b_t,c_t) \not\in \{2ab \in [1-4\lambda/5,1 - \lambda/ 8], |a^2 + b^2 + c| \leq \lambda / 4, a^2 + b^2 \leq 32 \}$, which means that $\|\nabla \ell(a_t,b_t,c_t)\|^2 \geq \lambda^2 (2a_tb_t) / 64 \geq \lambda^4 / 64$.

Thus, $\ell(a_{t+1},b_{t+1},c_{t+1}) \leq \ell(a_t,b_t,c_t) - \alpha \lambda^4 / 128$ for all $t \in \{0,\ldots,T-1\}$ by smoothness. So $\ell(a_T,b_T,c_T) \leq 1 - \lambda - T\alpha \lambda^4 / 128 < 0$, which is a contradiction. This proves the lemma.
\end{proof}

\paragraph{Once loss is at most $1/2$, we reach a loss of at most $\lambda / 2 - \lambda^2 / 50$ pretty quickly}

\begin{lemma}
If $\ell(a,b,c) \leq 1/2$, then $2ab \geq 1/10$.
\end{lemma}
\begin{proof}
Since $\ell(a,b,c) \geq (2ab - 1)^2$.
\end{proof}

\eb{Needs $4\lambda \alpha \leq 1/864$}
\begin{lemma}\label{lem:fracdecreases}
If $(a_t,b_t,c_t) \in \{2ab \in [1-4\lambda/5,1 - \lambda/ 8], |a^2 + b^2 + c| \leq \lambda / 4, a^2 + b^2 \leq 32 \}$ and $a_t \geq b_t$, then
\begin{align*}
0 \leq (\frac{a_{t+1}}{b_{t+1}} - 1) \leq (\frac{a_t}{b_t} - 1) \cdot (1 - \lambda \alpha / 96)
\end{align*}
\end{lemma}
\begin{proof}
For ease of notation, let $\kappa = 2(2a_t b_t - 1)$ and $\eta = 2(a_t^2 + b_t^2 + c_t)$. Note that $\kappa \in [-2\lambda, -\lambda /4]$ and $|\eta| \leq \lambda / 2$. Then
\begin{align*}
\frac{a_{t+1}}{b_{t+1}} &= \frac{a_t - \alpha(\lambda a_t + \kappa b_t + \eta a_t)}{b_t - \alpha (\lambda b_t + \kappa a_t + \eta b_t)} \\
&= \frac{(1 - \alpha(\lambda + \eta))a_t - \alpha \kappa b_t}{(1 - \alpha(\lambda + \eta))b_t - \alpha \kappa a_t}
\end{align*}
From the above expression it is clear that $1 \leq \frac{a_{t+1}}{b_{t+1}} \leq \frac{a_t}{b_t}$. Defining $\tau = -\frac{\alpha \kappa}{1 - \alpha(\lambda + \eta)}$, we may write
\begin{align*}
\frac{a_{t+1}}{b_{t+1}} /  \frac{a_t}{b_t}&= \frac{1 - \frac{\alpha \kappa}{1 - \alpha(\lambda + \eta)} b_t (b_t / a_t)}{1 - \frac{\alpha \kappa}{1 - \alpha(\lambda + \eta)} a_t (a_t / b_t)} \\
 &=\frac{1 + \tau b_t (b_t / a_t)}{1 + \tau a_t (a_t / b_t)}
\end{align*}
It is clear that this quantity is at most 1, since $\frac{a_{t+1}}{b_{t+1}} \leq \frac{a_t}{b_t}$. We now prove that it is bounded away from $1$.
\begin{align*}
\frac{1 + \tau b_t (b_t / a_t)}{1 + \tau a_t (a_t / b_t)} - 1 &= \frac{1 + \tau b_t (b_t / a_t) - (1 + \tau a_t (a_t / b_t))}{1 + \tau a_t (a_t / b_t)} \\
&= \frac{\tau b_t (b_t / a_t) - \tau a_t (a_t / b_t)}{1 + \tau a_t (a_t / b_t)} \\
&= \tau \frac{b_t (b_t / a_t) - a_t (a_t / b_t)}{1 + \tau a_t (a_t / b_t)} \\
& \geq \frac{b_t (b_t / a_t) - a_t (a_t / b_t)}{1 + 864\tau}
\end{align*}
where the last line is since $a_t^2 + b_t^2 \leq 32$ and $2a_t b_t \geq 1 - \lambda \geq 1/2$, which imply $a_t \leq 6$ and therefore $b_t \geq 1/24$. As a result $a_t (a_t / b_t) \leq 864$.
So since $\tau \leq 1 / 864$ because $\tau \leq 2\lambda \alpha / (1 - \alpha(\lambda + \lambda / 2)) \leq 4\lambda \alpha \leq 1/864$.
\begin{align*}
\frac{1 + \tau b_t (b_t / a_t)}{1 + \tau a_t (a_t / b_t)} - 1 & \geq \tau\frac{ b_t (b_t / a_t) - a_t (a_t / b_t)}{2} \\
&\geq \tau b_t \frac{(b_t / a_t) - (a_t / b_t)}{2}.
\end{align*}
So
\begin{align*}
\frac{a_{t+1}}{b_{t+1}} &\leq \frac{a_t}{b_t}( 1 - \tau b_t \frac{(a_t / b_t) - (b_t / a_t)}{2}) \\
&\leq \frac{a_t}{b_t} - (\tau b_t / 2) ((\frac{a_t}{b_t})^2 - 1) \\
&\leq \frac{a_t}{b_t} - (\tau b_t) (\frac{a_t}{b_t} - 1)
\end{align*}
So
\begin{align*}
\frac{a_{t+1}}{b_{t+1}} - 1 &\leq (\frac{a_t}{b_t} - 1)(1 - \tau b_t) \\
&\leq (\frac{a_t}{b_t} - 1)(1 - \tau / 24)
\end{align*}
Finally, $\tau \geq (\lambda \alpha / 4) / (1 + \alpha (\lambda + \lambda / 2)) \geq \lambda \alpha / 8$.

\end{proof}

\begin{lemma}
If $a_0,b_0,c_0$ is such that $\ell(a_0,b_0,c_0) \leq 1/2$, then $\ell(a_T,b_T,c_T) < \lambda/2 - \lambda^2 / 50$ for some $T = \Theta(\log(1/\lambda) / (\lambda^3 \alpha^2))$
\end{lemma}
\begin{proof}
We have $\ell(a_t,b_t,c_t) \leq \ell(a_0,b_0,c_0) \leq 1/2$ for all $t \geq 0$. We must have that for each $t \geq 0$ either $(a_t,b_t,c_t) \in \{2ab \in [1-4\lambda/5,1 - \lambda/ 8], |a^2 + b^2 + c| \leq \lambda / 4, a^2 + b^2 \leq 32 \}$, or $\|\nabla \ell(a_t,b_t,c_t)\|^2 \geq \min(\lambda^2 / 64, (2ab)\lambda^2 / 8) \geq \lambda^2 / 80$, since $2ab \geq  1/10$ by the previous lemma.

If $\|\nabla \ell(a_t,b_t,c_t)\|^2 \geq \lambda^2 / 80$, then $\ell(a_{t+1},b_{t+1},c_{t+1}) \leq \ell(a_t,b_t,c_t) - \alpha \lambda^2 / 160$. Therefore, let $S \subset \{0,\ldots,T-1\}$ be the time steps $S = \{t : \|\nabla \ell(a_t,b_t,c_t)\|^2 \geq \lambda^2 / 80\}$ where the gradient is lower-bounded by $\lambda^2 / 80$. We may assume without loss of generality that $|S| \leq 80 / (\alpha \lambda^2)$, or else $\ell(a_T,b_T,c_T) \leq 0$. By pigeonhole principle, there must be some interval $[T_1,T_2]$ of length $T_2 - T_1 \geq (|T| - |S|) / (|S| + 1) \geq  \geq \Omega(\log(1/\lambda) / (\lambda \alpha))$ such that $(a_t,b_t,c_t) \in \{2ab \in [1-4\lambda/5,1 - \lambda/ 8], |a^2 + b^2 + c| \leq \lambda / 4, a^2 + b^2 \leq 32 \}$ for all $t \in [T_1,T_2]$. Suppose without loss of generality we have $a_{T_1} \geq b_{T_1}$. By Lemma~\ref{lem:fracdecreases}, we must have $0 \leq \frac{a_{T_2}}{b_{T_2}} - 1 \leq (\frac{a_{T_1}}{b_{T_1}} - 1)(1 - \lambda \alpha / 96)^{T_2 - T_1}$. Since $a_{T_1}^2 + b_{T_1}^2 \leq 32$ and $2a_{T_1} b_{T_1} \geq 1/2$, it holds that $a_{T_1} \leq 6$ and $b_{T_1} \geq 1/24$, so $\frac{a_{T_1}}{b_{T_1}} \leq 864$. So $0 \leq \frac{a_{T_2}}{b_{T_2}} - 1 \leq (863)(1 - \lambda \alpha / 96)^{T_2 - T_1} \leq \lambda / 100$ since $T_2 - T_1 \geq \Omega(\log(1/\lambda) / (\lambda \alpha))$.

From this, it holds that \begin{align*}\ell(a_{T_2},b_{T_2},c_{T_2}) &= \frac{\lambda}{2}(a_{T_2}^2 + b_{T_2}^2) + \frac{1}{2}(2a_{T_2}b_{T_2} - 1)^2 + \frac{1}{2}(a_{T_2}^2 + b_{T_2}^2 + c_{T_2})^2 \\
&\leq \frac{\lambda}{2}(a_{T_2}^2 + b_{T_2}^2) + \frac{1}{2}(2a_{T_2}b_{T_2} - 1)^2 + \frac{1}{2}(\lambda / 4)^2 \\
&\leq \frac{\lambda}{2}(a_{T_2} b_{T_2} (1/(1 + \lambda / 100) + (1 + \lambda / 100)) + \frac{1}{2}(2a_{T_2}b_{T_2} - 1)^2 + \lambda^2 / 32 \\
&\leq \frac{\lambda}{2}(2a_{T_2} b_{T_2}) + \frac{1}{2}(2a_{T_2}b_{T_2} - 1)^2 + \frac{\lambda^2(a_{T_2}b_{T_2})}{200} + \lambda^2 / 32 \\
&\leq \frac{\lambda}{2}(2a_{T_2} b_{T_2}) + \frac{1}{2}(2a_{T_2}b_{T_2} - 1)^2 + \frac{\lambda^2}{400} + \lambda^2 / 32, & \mbox{since $a_{T_2} b_{T_2} \leq 1/2$} \\
&\leq \max(\frac{\lambda}{2}(1 - 4\lambda / 5) + \frac{1}{2}(4\lambda / 5)^2, \frac{\lambda}{2}(1 - \lambda / 8) + \frac{1}{2}(\lambda / 8)^2) + \frac{\lambda^2}{400} + \lambda^2 / 32, & \mbox{ since $2a_{T_2}b_{T_2} \in [1-4\lambda/5,\lambda/8]$} \\
&\leq \max(\frac{\lambda}{2} - 4\lambda^2 / 10 + 16\lambda^2 / 50, \frac{\lambda}{2} - \lambda^2 / 16 + \lambda^2 / 128) + \frac{\lambda^2}{400} + \lambda^2 / 32 \\
&\leq \frac{\lambda}{2} - \lambda^2 / 16 + \lambda^2 / 128 + \frac{\lambda^2}{400} + \lambda^2 / 32 \\
&\leq \frac{\lambda}{2} - \lambda^2 / 16 + \lambda^2 / 128 + \frac{\lambda^2}{400} + \lambda^2 / 32 \\
&< \lambda / 2 - \lambda^2 / 50
\end{align*}

\end{proof}

\paragraph{Once loss is at most $\lambda/2 - \lambda^2 / 50$, we make geometrically-fast progress to the optimum}

\begin{lemma}
If $\ell(a_0,b_0,c_0) < \lambda / 2 - \lambda^2 / 50$ then $2ab \in [1 - O(\lambda), 1 - \Omega(\lambda)]$.
\end{lemma}
\begin{proof}
Straightforward.
\end{proof}

\begin{lemma}
If $\ell(a_0,b_0,c_0) < \lambda / 2 - \lambda^2 / 50$, then $(\frac{a_1}{b_1} - 1)) \leq (\frac{a_0}{b_0} - 1) \cdot (1 - \Omega(\lambda \alpha))$.
\end{lemma}
\begin{proof}
Similar to a previous lemma. \eb{fill in}
\end{proof}

\begin{lemma}
If $\ell(a_0,b_0,c_0) < \lambda / 2 - \lambda^2 / 50$, then after $T = \poly(\log(1/\delta),1/\alpha,1/\lambda)$ iterations we have $\ell(a_T,b_T,c_T) \leq \delta$.
\end{lemma}
\begin{proof}
Simple, using the previous lemma to ensure that $|a_t/b_t| \in [1-o(\delta),1+o(\delta)]$ for all $t \geq T'$ for some $T' = \poly(\log(1/\delta),1/\alpha,1/\lambda)$. At that point the loss function is for all intents and purposes strictly convex. \eb{formalize}
\end{proof}

\subsection{Left to write up}

\begin{itemize}
    \item $\sgn(a_0) \neq \sgn(b_0)$. Reason about relative increase in $a_0$ to $b_0$ in a small enough number of iterations that you can ``catapult'' into the $\sgn(a_0) = \sgn(b_0)$ region. The key property is that you need $|a_0 / b_0|$ to be bounded away from 0, even if by only an exponentially-small amount. This is guaranteed with exponentially-high probability at initialization.
    \item With noisy inputs -- most of the analysis is the same: use that the gradients are $O(\delta\lambda)$ close, so the initial phases work the same way -- until we reach the geometric convergence regime, where we stop at a $O(\delta)$-approximate solution.
\end{itemize}

\section{Training the neuron with noise}
Suppose that we are given access to an approximate gradient oracle $\gt(a,b,c)$ that evaluates $\nabla \ell(a,b,c)$ up to error $\|\gt(a,b,c) - \nabla \ell(a,b,c)\| \leq \eps$. Then we prove that gradient descent using the gradient oracle $\gt$ will still in arriving to a solution with small noise.

\begin{lemma}
The high-change regions, where $\|\nabla \ell\| \geq 4\eps$ still see major decrease in the loss $\ell$ (easy -- same calculations as before, same smoothness as before).
\end{lemma}

\begin{lemma}
The low-change regions, where $\|\nabla \ell \leq 4\eps$ are trickier, but can still be handled. They are tricky because the loss $\ell$ may not be decreasing monotonically. However, by the smoothness of $\ell$ and $\ellt$, and the fact that our empirical dataset is large enough, we may prove that $\ell$ and $\ellt$ are additively-close. Since $\ellt$ does not increase, this is good enough to do our analysis.
\begin{itemize}
    \item The region where the loss goes from $1 - \lambda$ to $1/2$.
    
    \item The region where the loss goes from $1/2$ to $\leq \lambda - \lambda^2 / 50$. Also tricky, because the loss may not be decreasing monotonically. However, we may still easily prove that the ratio of $a$ and $b$ tends to 1. And we may also easily prove that we accumulate loss slowly if on the particular step we are focused on the ratio, and not losing loss quickly.
    
    \item The final region, with the loss going to 
\end{itemize}
\end{lemma}


\section{Smoothness and gradient evaluation properties in the wild}
We now state and prove the main local update lemma. Suppose that $f_1(x)$ and $f_2(x)$ are such that $f_1(x) = x_{S_1} + h_1(x)$, $f_2(x) = x_{S_2} + h_2(x)$ where $|h_1(x)|, |h_2(x)| \leq \epsilon$ for all $x$. Then if $x_{S_1}x_{S_2}$ is a monomial in the target function, training a neuron with inputs $f_1$ and $f_2$ will approximately learn $x_{S_1} x_{S_2}$ up to $O(\epsilon)$ error. This can be stated more simply with a few more definitions:

\begin{definition}
We say that a function $f(x)$ is a $\eps$-approximation of $g(x)$ if $|f(x) - g(x)| \leq \eps$ for all $x$.
\end{definition}


Let $0 < \lambda < 1$ be the $L^2$ regularization parameter.
Define the noiseless loss function. This arises when we are trying to learn exactly $x_{S_1} x_{S_2}$ (no other monomials in the sum), and $f_1(x)$ and $f_2(x)$ are exact.
\begin{definition}[Noiseless loss function]
$\ellt(a,b,c) = \frac{1}{2}(2ab - 1)^2 + \frac{1}{2}(a^2 + b^2 + c)^2 + \frac{\lambda}{2} (a^2 + b^2)$
\end{definition}
Define the noisy loss function. This arises when we are trying to learn $g(x)$ such that $\hat{g}(S_1 \Delta S_2) = 1$ and $|\hat{g}(\emptyset)| \leq $ and $|g(x)| \leq M$ for all $x$.
\begin{definition}[True loss function]
The true loss is
\begin{align*}
\ell(a,b,c) &= \EE_x [\frac{1}{2}(f(x) - g(x))^2 + (\lambda / 2)(a^2 + b^2)] \\
&= \EE_x [\frac{1}{2}((a f_1(x) + b f_2(x))^2 + c - g(x))^2 + (\lambda / 2)(a^2 + b^2)]
\end{align*}
\end{definition}
Thus, \begin{align*}
\pd{\ell}{w} &= \EE_x[ \pd{}{w} \frac{1}{2}(((a f_1(x) + b f_2(x))^2 + c - g(x))^2 + (\lambda / 2)(a^2 + b^2))],
\end{align*}
so
\begin{align*}
\pd{\ell}{a} &= \EE_x[((a f_1(x) + b f_2(x))^2 + c - g(x))(2(a f_1(x) + b f_2(x)) f_1(x)) + \lambda a]
\pd{\ell}{b} &= \EE_x[((a f_1(x) + b f_2(x))^2 + c - g(x))(2(a f_1(x) + b f_2(x)) f_2(x)) + \lambda b]
\pd{\ell}{c} &= \EE_x[((a f_1(x) + b f_2(x))^2 + c - g(x))].
\end{align*}
so letting $\Delta(x;a,b,c) = ((a f_1(x) + b f_2(x))^2 + c - g(x))$, we can rewrite this as
\begin{align*}
\pd{\ell}{a} &= \EE_x[\Delta(x;a,b,c)(2(a f_1(x) + b f_2(x)) f_1(x)) + \lambda a]
\pd{\ell}{b} &= \EE_x[\Delta(x;a,b,c)(2(a f_1(x) + b f_2(x)) f_2(x)) + \lambda b]
\pd{\ell}{c} &= \EE_x[\Delta(x;a,b,c)].
\end{align*}


We prove that $\ell$ is smooth when $a,b,c$ are stuck in a box throughout training, which is the case because of the $L^2$ regularization:
\begin{lemma}
$\|\nabla^2 \ell(a,b,c)\| \leq \max(|a|,|b|,|c|)^2$.
\end{lemma}
\begin{proof}
\eb{complete}
\begin{align*}
|\frac{\partial^2 \ell}{\partial a^2}| &= |\EE_x[\pd{\Delta(x;a,b,c)}{a} (2f_1(x))(a f_1(x) + b f_2(x)) + (\Delta(x;a,b,c))(2 (f_1(x))^2) + \lambda]| \\
&\leq |\EE_x[\pd{\Delta(x;a,b,c)} (2f_1(x))(a f_1(x) + b f_2(x))]| + |\EE_x[(\Delta(x;a,b,c))(2 (f_1(x))^2)]| + \lambda \\
&\leq \eb{polynomial bound, and complete bounds that have been commented out}
\end{align*}
\end{proof}

We prove that $\nabla \ell$ is close to $\nabla \ellt$ in additive terms:
\begin{lemma}
$|\pd{\ell}{a} - \pd{\ellt}{a}| \leq |\hat{g}(\emptyset)| \cdot |2a| + |1 - \hat{g}(S_1 \Delta S_2)| \cdot |2b| + \epsilon \poly(M,\|w\|)$, and
$|\pd{\ell}{b} - \pd{\ellt}{b}| \leq |\hat{g}(\emptyset)| \cdot |2b| + |1 - \hat{g}(S_1 \Delta S_2)| \cdot |2a| + \epsilon \poly(M,\|w\|)$, and
$|\pd{\ell}{c} - \pd{\ellt}{c}| \leq |\hat{g}(\emptyset)| + \epsilon \poly(M,\|w\|)$
\end{lemma}
\begin{proof}
\begin{align*}
|\pd{\ell}{a} - \pd{\ellt}{a}| &= |\lambda a + \EE_x[\Delta(x;a,b,c)(2(a f_1(x) + b f_2(x)) f_1(x)) - (\lambda a + (2ab - 1)(2b) + (a^2 + b^2 + c)(2a))]| \\
&= |\EE_x[\Delta(x;a,b,c)(2(a f_1(x) + b f_2(x)) f_1(x))] - ((2ab - 1)(2b) + (a^2 + b^2 + c)(2a))|
\end{align*}
And
\begin{align*}
\EE_x[\Delta(x;a,b,c)(2(a f_1(x) + b f_2(x)) f_1(x))] &= \EE_x[((a f_1(x) + b f_2(x))^2 + c - g(x))(2(a f_1(x) + b f_2(x)) f_1(x))] \\
&= \EE_x[((a (x_{S_1} + h_1(x)) + b (x_{S_2} + h_2(x)))^2 + c - g(x))(2(a (x_{S_1} + h_1(x)) + b (x_{S_2} + h_2(x))) (x_{S_1} + h_1(x)))] \\
&= \EE_x[((a (x_{S_1} + h_1(x)) + b (x_{S_2} + h_2(x)))^2 + c - g(x))(2(a (1 + 2x_{S_1} h_1(x) + h_1(x)^2) + b (x_{S_1} x_{S_2} + x_{S_1} h_2(x) + x_{S_2} h_1(x) + h_1(x) h_2(x)))]
\end{align*}

\begin{align*}
\ell(w) &= \frac{\lambda}{2}(a^2 + b^2) + \frac{1}{2}\EE_x[((a (x_{S_1} + h_1(x)) + b (x_{S_2} + h_2(x)))^2 + c - g(x))^2] \\
&= \frac{\lambda}{2}(a^2 + b^2) + \frac{1}{2}\EE_x[((a^2 (x_{S_1} + h_1(x))^2 + b^2 (x_{S_2} + h_2(x))^2 + 2ab (x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) + c - g(x))^2] \\
&= \frac{\lambda}{2}(a^2 + b^2) + \frac{1}{2}\EE_x[((a^2 + b^2 + 2ab x_{S_1} x_{S_2} + c - g(x) + a^2 ((x_{S_1} + h_1(x))^2 - 1) + b^2 ((x_{S_2} + h_2(x))^2 - 1) + 2ab (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}))^2] \\
&= T_1 + T_2 + T_3,
\end{align*}
where
\begin{align*}
T_1 &= \frac{\lambda}{2}(a^2 + b^2) + \frac{1}{2}\EE_x[(a^2 + b^2 + 2ab x_{S_1} x_{S_2} + c - g(x))^2], \\
T_2 &= \frac{1}{2}\EE_x[2(a^2 + b^2 + 2ab x_{S_1} x_{S_2} + c - g(x))(a^2 ((x_{S_1} + h_1(x))^2 - 1) + b^2 ((x_{S_2} + h_2(x))^2 - 1) + 2ab (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}))], \\
T_3 &= \frac{1}{2}\EE_x[(a^2 ((x_{S_1} + h_1(x))^2 - 1) + b^2 ((x_{S_2} + h_2(x))^2 - 1) + 2ab (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}))^2].
\end{align*}

By Parseval's identity:
\begin{align*}
T_1 &= \frac{\lambda}{2}(a^2 + b^2) + \frac{1}{2}(a^2 + b^2 + c - \hat{g}(\emptyset))^2 + \frac{1}{2}(2ab - \hat{g}(S_1 \Delta S_2))^2 + \frac{1}{2}\sum_{S \subset [n] \sm \{\emptyset, S_1 \Delta S_2\}} \hat{g}(x)^2
\end{align*}
So
\begin{align*}
\pd{T_1}{a} &= \lambda a + (a^2 + b^2 + c - \hat{g}(\emptyset))(2a) + (2ab - \hat{g}(S_1 \Delta S_2))(2b)
\end{align*}
and
\begin{align*}
\pd{T_1}{c} &= a^2 + b^2 + c - \hat{g}(\emptyset)
\end{align*}
So
\begin{align*}
|\pd{T_1}{a} - \pd{\ellt}{a}| &= |- \hat{g}(\emptyset)(2a) + (1 - \hat{g}(S_1 \Delta S_2))(2b)| \\
&\leq |\hat{g}(\emptyset)| \cdot |2a| + |1 - \hat{g}(S_1 \Delta S_2)| \cdot |2b|
\end{align*}
Similarly,
\begin{align*}
|\pd{T_1}{b} - \pd{\ellt}{b}| &= |- \hat{g}(\emptyset)(2b) + (1 - \hat{g}(S_1 \Delta S_2))(2a)| \\
&\leq |\hat{g}(\emptyset)| \cdot |2b| + |1 - \hat{g}(S_1 \Delta S_2)| \cdot |2a|
\end{align*}
And
\begin{align*}
|\pd{T_1}{c} - \pd{\ellt}{c}| &= |\hat{g}(\emptyset)|
\end{align*}

Finally, we prove that $\pd{T_2 + T_3}{w}$ is quite small:
Let \begin{align*}
r_1(x) &=  (a^2 + b^2 + 2ab x_{S_1} x_{S_2} + c - g(x)) \\
r_2(x) &= (a^2 ((x_{S_1} + h_1(x))^2 - 1) + b^2 ((x_{S_2} + h_2(x))^2 - 1) + 2ab (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}))
\end{align*}
and recall that $T_2 = \EE_x[r_1r_2]$.
\begin{align*}
\pd{T_2}{w} &= \EE_x[\pd{r_1}{w} r_2 + r_1 \pd{r_2}{w}]
\end{align*}
And 
\begin{align*}
\pd{r_1}{a} &= 2a + 2b x_{S_1} x_{S_2} \\
\pd{r_1}{b} &= 2b + 2a x_{S_1} x_{S_2} \\
\pd{r_1}{c} &= 1 \\
\pd{r_2}{a} &= 2a ((x_{S_1} + h_1(x))^2 - 1) + 2b (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}) \\
\pd{r_2}{b} &= 2b ((x_{S_2} + h_2(x))^2 - 1) + 2a (((x_{S_1} + h_1(x))(x_{S_2} + h_2(x))) - x_{S_1} x_{S_2}) \\
\pd{r_2}{c} &= 0
\end{align*}
And
\begin{align*}
|\pd{r_2}{a}| &\leq |2a| \cdot (2 |h_1(x)| + |h_1(x)|^2) + |2b| \cdot (|h_1(x)| + |h_2(x)| + |h_1(x)||h_2(x)|) \leq 5\epsilon(|a| + |b|)\\
|\pd{r_2}{b}| &\leq |2b| \cdot (2 |h_2(x)| + |h_2(x)|^2) + |2b| \cdot (|h_1(x)| + |h_2(x)| + |h_1(x)||h_2(x)|) \leq 5\epsilon(|a| + |b|)
\end{align*}
And
\begin{align*}
r_1(x) \leq O(\max(|a|,|b|)^2)
r_2(x) \leq O(\epsilon \max(|a|,|b|)^2)
\end{align*}
So
\begin{align*}
|\pd{T_2}{a}| &= |\EE_x[\pd{r_1}{a} r_2 + r_1 \pd{r_2}{w}]| \leq O(\epsilon (\max(|a|,|b|)^3 + \max(|a|,|b|) (M + |c| + |a|^2 + |b|^2))) \\
|\pd{T_2}{b}| &\leq O(\epsilon (\max(|a|,|b|)^3 + \max(|a|,|b|) (M + |c| + |a|^2 + |b|^2))) \\
|\pd{T_2}{c}| &\leq O(\epsilon \max(|a|,|b|)^3)
\end{align*}
Similarly, $T_3 = \frac{1}{2}\EE_x[r_2(x)^2]$
\begin{align*}
|\pd{T_3}{a}| &= |\EE_x[r_2(x) \pd{r_2(x)}{a}]| \leq O(\epsilon^2 \max(|a|,|b|)^3) \\
|\pd{T_3}{b}| &\leq O(\epsilon^2 \max(|a|,|b|)^3) \\
|\pd{T_3}{c}| &= 0
\end{align*}
So
\begin{align*}
|\pd{\ell}{a} - \pd{\ellt}{a}| \leq |\pd{T_1}{a} - \pd{\ellt}{a}| + |\pd{T_2}{a}| + |\pd{T_3}{a}| \leq |\pd{T_1}{a} - \pd{\ellt}{a}| + \eps \cdot \poly(M,|a|,|b|,|c|) \\
|\pd{\ell}{c} - \pd{\ellt}{c}| \leq |\pd{T_1}{c} - \pd{\ellt}{c}| + |\pd{T_2}{c}| + |\pd{T_3}{c}| \leq |\pd{T_1}{c} - \pd{\ellt}{c}| + \eps \cdot \poly(M,|a|,|b|,|c|)
\end{align*}
Combining this with the above inequalities proves the lemma.
\end{proof}

The fact that $\pd{\ell}{w}$ is close to $\pd{\ellt}{w}$ means that if $\nabla \ellt$ is large, then $\nabla \ell$ is quite aligned to $\nabla \ell$. This means that in all of the easy regions of the analysis for $\ellt$ where we can lower-bound the loss decrease by an inverse polynomial, we automatically obtain a similar bound for $\ellt$. In particular, it is clear that $\ell$ and $\ellt$ are essentially $\eps$-close (with some extra polynomial factors). This means that we can reason that at most $\lambda^2 - \lambda / 50$ loss is reached at some point (plus the loss from terms that have nothing to do with the $S_1 \Delta S_2$ or $\emptyset$ coefficients. In this region, again we can prove that $a_t$ and $b_t$ approach a ratio of 1 exponentially-quickly, as long as the error in the gradient is upper-bounded. So everything is OK with this analysis -- although it should be written up. We can prove that after some polynomial number of iterations, the ratio of $a_t$ to $b_t$ will be quite close.

\begin{theorem}[Local update theorem]
If we set $a_0,b_0,c_0 \sim \cN(0,1)$, then there is a constant $C$ such that for any $0 < \delta < 1/2$ and $T \geq (\log(1/\delta),1/\alpha,1/\lambda)^C$, we have the bound $$\ell(a_t,b_t,c_t) \leq \delta$$ with probability $\geq 1 - \delta$.
\end{theorem}
}

\begin{lemma}

\end{lemma}

{\color{gray} 
\section{Neural network proofs}
\subsection{Setup}
\paragraph{Architecture}
Neural net on $\ell$ layers, width $w$. $n$ input neurons $(0,1),\ldots,(0,n)$, where neuron $(0,j)$ computes $f_{0,j}(x) = x_j$. Edge set $E$. Let $\inedges(i,j)$ denote edges in $E$ that go into neuron $(i,j)$.
Neuron $(i,j)$ for $i \in [\ell]$, $j \in [w]$ computes $f_{i,j}(x) = \left(\sum_{e = ((i',j'),(i,j)) \in \inedges(i,j)} A_e f_{i',j'}(x) \right)^2 + b_{i,j}$. Here $A_e$ is the weight of edge $e$, and $b_{i,j}$ is a bias term for the neuron. The output of the neural net is $f(x) = \sum_{(i,j) \in [\ell] \times [w]} f_{i,j}(x)$.

We set $E$ so that every $((0,j),(i',j'))$ is in $E$ independently with probability $p$ for all $j \in [n]$ and $i' \in [\ell], j' \in [w]$. Also, every $((i,j),(i+1,j'))$ is in $E$ independently with probability $p$ for all $i \in [\ell-1], j,j' \in [w]$.

\subsection{Loss function}

Let the loss function be the mean-squared-error between the output $f$ of the network and an $s$-sparse $M$-HBF $g$.
\begin{equation}
    \loss(A,b) = \EE_{x \sim \{-1,1\}^n} \loss(A,b,x) = \EE_{x \sim \{-1,1\}^n} \frac{1}{2}(f(A,b,x) - g(x))^2
    \label{eq:loss}
\end{equation}



\paragraph{Training}
We train to learn a hierarchical boolean function (HBF) $g$ by running Algorithm~\ref{alg:cd}.

Let $\nu = (i,j)$ be a neuron.
Let $b_{\nu}^{(t,t')}$ and $A_e^{(t,t')}$ denote the bias and weights respectively, over time. 
Similarly, $f^{(t,t')}$ is the function computed at time $(t,t')$. Here $t \in [\Tout]$ keeps track of the outer iteration, and $t' \in \{0,\ldots,\Tin\}$ keeps track of the inner iteration.

At the beginning of the $t$th outer loop iteration, $f^{(t,0)}$ is the function we start with. $f^{(t,1)}$ is the function after perturbing $f^{(t,0)}$'s weights randomly, and $f^{(t,\Tin)}$ is the function at the end of all of the \ref{step:cdupdate} iterations. We write $f^{(t,\Tin)} = f^{(t+1,0)}$.

\begin{algorithm}\SetAlgoLined\DontPrintSemicolon
    \KwIn{
    Blackbox access to $g$, an $s$-sparse HBF
    }
    \KwOut{trained weights $A$, biases $b$ for the neural net}
    
    \BlankLine
    
    Initialize $b_{i,j} = 0$ for all $(i,j) \in [\ell] \times [w]$, and $A_e = 0$ for all $e \in E$.
    
    \For{$t = 1$ to $\Tout$}{
        Pick a neuron $(i,j) \in [\ell] \times [w]$ uniformly at random. \label{step:cdpickneuron}
    
        \tcp{To avoid saddle points during optimization, perturb neuron weights}
        $b_{i,j} \gets b_{i,j} +  \mathrm{Unif}[-\pnoise, \pnoise]$, and $A_e \gets A_e + \mathrm{Unif}[-\pnoise, \pnoise]$ for $e \in \inedges(i,j)$.\label{step:cdperturbweights}
        
        \tcp{Train neuron with GD on the neuron parameters}
        \For{$t' = 1$ to $\Tin$}{
        Simultaneously update $b_v \gets b_v - \eta \pd{\ell}{b_v}$ and $A_e \gets A_e - \eta \pd{\ell}{A_e}$ for all  $e = (u,v) \in E$  \label{step:cdupdate}
         }
    }
    \caption{Coordinate descent}
\label{alg:cd}
\end{algorithm}

\paragraph{Helpful notation throughout training}
We will use $\Delta^{(t,t')} = f^{(t,t')} - g$ to denote the difference between the function trained so far and the true function.

\subsection{Result}


\begin{theorem}\label{thm:cdguarantee}
Let $g$ be an $s$-sparse $M$-HBF.
If $\Tout \geq $, $\Tin \geq $, $\eps < $, $ < p < $, then Algorithm~\ref{alg:cd} will learn $g$ up to $< $ error.
\end{theorem}

The proof is based on several lemmas proved in the subsections below. First, in Section~\ref{ssec:invariants} we define certain basic invariants that will be maintained throughout training. Second, in Section~\ref{ssec:localupdates} we reason about each coordinate descent step affects these invariants. Finally, in Section~\ref{ssec:globaltrajectory} we formally prove Theorem~\ref{thm:cdguarantee} based on the results of Sections~\ref{ssec:invariants} and \ref{ssec:localupdates}.

\subsection{Invariants}\label{ssec:invariants}

In this subsection, we present several invariants that we will later prove are maintained during the training procedure of Algorithm~\ref{alg:cd}. In order to present these invariants, we must define ``blank'' neurons and ``active'' neurons. First, we say that a neuron is blank if it computes the zero function identically, and also all input and output edges have zero weight:
\begin{definition}
A neuron $(i,j)$ is {\em blank} if $f_{i,j}(x) = 0$, $b_{i,j} = 0$, and $A_e = 0$ for all $e \in \inedges(i,j) \cup \outedges(i,j)$.
\end{definition}

Second, we say that a neuron is active if it is well-excited by any input to the neural network.
\begin{definition}[Active neuron]
A neuron $(i,j)$ is {\em active} if $|f_{i,j}(x)| \geq 1/2$ for all $x$.
\end{definition}

The first invariant that we maintain during training is that every neuron is either blank or active:
\begin{definition}[Invariant 1: blank/active] \label{def:blankactiveinvariant}
The {\em Blank/Active Invariant} states that: every time that we reach step~\ref{step:pickneuron} of training, every neuron $(i,j)$ is either blank or active.
\end{definition}

The second invariant is that every active neuron computes some monomial up to a good approximation. To formalize this, let us first define the relevant notion of approximation:
\begin{definition}[Almost-sure approximation]
Two functions $h_1, h_2 : \{-1,1\}^n \to \RR$ are $\delta$-approximately close if, for all $x \in \{-1,1\}^n$, $$|h_1(x) - h_2(x)| \leq \delta.$$
\end{definition}

Using this notion of approximation, we can write what it means for a neuron to approximate a monomial well. 
\begin{definition}
A neuron $(i,j)$ computes a $\delta$-approximate monomial if there is some $s \in \{-1,1\}$, $S \subset [n]$ such that $h_1(x) = f_{i,j}(x)$ and $h_2(x) = s x_S$ are $\delta$-close. We say that $s x_S$ is the monomial that $(i,j)$ approximates up to error $\delta$.
\end{definition}

\begin{definition}[Invariant 2: active neurons compute monomials] \label{def:approximatemonomialinvariant}
The {\em Approximate-Monomials Invariant} states that: on iteration $t$, when we hit step~\ref{step:pickneuron}, every active neuron computes a $\delta_t$-approximate monomial.
\end{definition}


The third invariant that we will show is that, at all times, every neuron has at most two active predecessors. This will essentially follow from the fact that (a) there is a small number of active neurons at any given point in time, and (b) the connectivity graph of the neural network is very sparse.
\begin{lemma}[Invariant 3: ]
For every neuron $(i,j)$, there are at most two predecessors that are active: i.e.,
$$|\{(i',j') : ((i',j'),(i,j)) \in \inedges(i,j) \mbox{ and } (i',j') \mbox{ is active}\}|.$$
\end{lemma}

The fourth invariant is that, each time we start the outer loop of training, or end the inner loop, the true function is learned without any bias.
\begin{definition}[Invariant 4: No-Bias Invariant] \label{def:nobiasinvariant}
$|\hat{\Delta^{(t,0)}}(\emptyset)| \ll \epsbiasthresh$ throughout training.
\end{definition}

\subsection{Local update lemmas}\label{ssec:localupdates}

In this section, we will prove several lemmas that will let us reason about how the invariants of the network change on each time that we run an iteration of the loop from steps~\ref{step:pickneuron} through \ref{step:round} of Algorithm~\ref{alg:cd}. For clarity, let us standardize the notation across the lemmas in this section. Let $(i,j)$ be the neuron picked at step~\ref{step:pickneuron} of Algorithm. Let the set of active predecessor neurons to $(i,j)$ at this step be $P = \{(i',j') : ((i',j'),(i,j)) \in \inedges(i,j) \mbox{ and } (i',j') \mbox{ is active}\}$.

\begin{definition}
We say that all invariants hold if the following invariants hold:
\begin{itemize}
    \item Blank/Active Invariant (Definition~\ref{def:blankactiveinvariant})
    \item Approximate-Monomial Invariant (Definition~\ref{def:approximatemonomialinvariant})
\end{itemize}
\end{definition}

The first lemma we prove states that if $(i,j)$ is blank and it has fewer than two active inputs, then $(i,j)$ is unchanged.
\begin{lemma}[Blank neurons with fewer than one active input are unchanged] 
Suppose that $(i,j)$ is blank and $|P| \leq 1$. Then after step~\ref{step:round}, $(i,j)$ remains blank.
\end{lemma}
\begin{proof}
First, write the expression for the function computed by neural network:
$f(x) = \sum_{i' \in [\ell], j' \in [w]} f_{i',j'}(x)$

Then, write the expression for the change created by perturbing the input weights to neuron $i,j$ and the bias $b_{i,j}$. For any edge $e \in \inedges(i,j)$, we have
$\frac{\partial f(x)}{\partial A_{e}} =  \sum_{i' \in [\ell], j' \in [w]} \frac{\partial f_{i',j'}(x)}{\partial A_e}$
For every neuron $(i',j')$ such that $(i',j')$ is an ancestor of $(i,j)$ we must have $\frac{\partial f_{i',j'}(x)}{\partial A_e} = 0$, because $f_{i',j'}$ does not depend on changes in $A_e$, which only affect downstream computation. As a result
$\frac{\partial f(x)}{\partial A_e} = \sum_{(i',j') \in [\ell] \times [w], \mbox{ downstream from } (i,j)} \frac{\partial f_{i',j'}}{\partial A_e}$.
Furthermore, for every neuron $(i',j')$ such that $(i',j')$ is a strict successor of $(i,j)$, since $A_{e'} = 0$ for all $e' \in \outedges(i,j)$, we must have $\frac{\partial f_{i',j'}(x)}{\partial f_{i,j}}$. We conclude that
$$\frac{\partial f(x)}{\partial A_e} = \frac{\partial f_{i,j}(x)}{\partial A_e}$$ for all $e \in \inedges(i,j)$.
By the same argument,
$$\frac{\partial f(x)}{\partial b_{i,j}} =  \sum_{i' \in [\ell], j' \in [w]} \frac{\partial f_{i',j'}(x)}{\partial b_{i,j}} = \frac{\partial f_{i,j}(x)}{\partial b_{i,j}}.$$

Recall that $f_{i,j}(x) = \sigma\left(\sum_{e'' = ((i'',j''),(i,j)) \in \inedges(i,j)} A_{e''} f_{i'',j''}(x) \right) + b_{i,j}$. Thus, for any $e' = ((i',j'),(i,j))$, it holds that
\begin{align*}
\frac{\partial f(x)}{\partial A_{e'}} &= \frac{\partial f_{i,j}(x)}{\partial A_{e'}} \\
&= \frac{\partial}{\partial A_{e'}}\left(\sigma\left(\sum_{e'' = ((i'',j''),(i,j)) \in \inedges(i,j)} A_{e''} f_{i'',j''}(x) \right) + b_{i,j}\right) \\
&= \sigma'\left(\sum_{e'' = ((i'',j''),(i,j)) \in \inedges(i,j)} A_e f_{i'',j''}(x) \right) \cdot f_{i',j'}(x)
\end{align*}
Similarly,
\begin{align*}
\frac{\partial f(x)}{\partial b_{i,j}} &= \frac{\partial f_{i,j}(x)}{\partial b_{i,j}} \\
&= 1.
\end{align*}

Now let us prove the lemma for the case $|P| = 0$. We will argue that GD does not change the monomial -- because there is no change in $f$ associated with changing the input weights. In this case, we have that $f_{i',j'}(x) = 0$ for all $(i',j')$ such that $((i',j'),(i,j)) \in \inedges(i,j)$. This implies that for any $e' \in \inedges(i,j)$ \begin{align*}
    \frac{\partial f(x)}{\partial A_{e'}} = 0
\end{align*}
This implies that if we look at the derivative of the loss from \eqref{eq:loss}:
$\loss(A,b) = \EE_{x \sim \{-1,1\}^n} \loss(A,b,x) = \EE_{x \sim \{-1,1\}^n} \frac{1}{2}(f(A,b,x) - g(x))^2$
for any $e' \in \inedges(i,j)$
\begin{align*}
    \pd{\loss(A,b)}{A_{e'}} &= \EE_{x \sim \{-1,1\}^n} \pd{}{A_{e'}} \frac{1}{2}(f(A,b,x) - g(x))^2 \\
    &= \EE_{x \sim \{-1,1\}^n} (f(A,b,x) - g(x)) \pd{}{A_{e'}} \left(f_{i,j}(x)\right) \\
    &= \EE_{x \sim \{-1,1\}^n} (f(A,b,x) - g(x)) \cdot 0 \\
    &= 0,
\end{align*}
where we have used that since all inputs are blank in fact the function computed by the network does not change with $A_{e'}$. Next, we note
\begin{align*}
    \pd{\loss(A,b)}{b_{i,j}} &= \EE_{x \sim \{-1,1\}^n} \pd{}{b_{i,j}} \frac{1}{2}(f(A,b,x) - g(x))^2 \\
    &= \EE_{x \sim \{-1,1\}^n} (f(A,b,x) - g(x)) \pd{}{b_{i,j}} \left(f_{i,j}(x)\right) \\
    &= \EE_{x \sim \{-1,1\}^n} (f(A,b,x) - g(x)) \cdot 1 \\
    &= \EE_{x \sim \{-1,1\}^n} (f(A,b,x) - g(x)),
\end{align*}
The reason that this helps us is because we can use it to prove that after a polynomial number of steps the bias will in fact be exponentially-small -- since the two functions were close before \ref{step:cdperturbweights}. Thus, after the round-off step~\ref{step:round}, the bias $b_{i,j}$ will be exponentially close to zero, and we will round it down to zero.
Let us go through the update equations. By the No-Bias invariant~\ref{def:nobiasinvariant}


If $|A| = 1$, then GD does not change the monomial, because we would just be learning an affine shift of the monomial corresponding to the active predecessor, and we cannot learn an affine shift that will be of any remotely close magnitude that it will not be shaved off by the rounding step, because the active predecessor $(i,j)$ corresponds to a monomial that is already very well approximated by the neural network (so $\hat{\Delta}(x_S) \in [-\delta_t,\delta_t]$ for that monomial), so the weights we will learn here will never be able to overcome the rounding threshold.
\end{proof}

\begin{lemma}[Blank neurons can be converted to active neurons if useful, and otherwise stay blank during training]
Suppose that $(i,j)$ is blank and $|A| = 2$, with $A = \{(i_1,j_1),(i_2,j_2)\}$. Also suppose that $(i,j)$ does not have any active successors. Furthermore, suppose neuron $(i_1,j_1)$ computes a $\delta_1$-approximation to $s_1 x_{S_1}$ and neuron $(i_2,j_2)$ computes a $\delta_2$-approximation to $s_2 x_{S_2}$. Then let $S = S_1 \Delta S_2$.
\begin{itemize}
    \item If $x_S$ is such that $|\hat{\Delta}(S)| \geq 1/2$, then after training $(i,j)$ computes a $(\delta_1 + \delta_2 + \eps)$-approximation to $x_S$ with probability at least $1/2$, and is blank otherwise.
    \item If $x_{S}$ is such that $|\hat{\Delta}(S)| \leq \eps$, then after training $(i,j)$ remains blank. 
\end{itemize}
\end{lemma}

\begin{lemma}[Active neurons are largely unchanged by repeated training]
Suppose that $(i,j)$ is active. Then training does not change $(i,j)$ too much?? And only lowers the error??? And does not hurt downstream monomial approximations? In fact, it should only help them.
\end{lemma}

\subsection{Maintaining global invariants}\label{ssec:globaltrajectory}

In this section, we prove Theorem~\ref{thm:cdguarantee} by proving that the global invariants defined in Section~\ref{ssec:invariants} are maintained. This will be done by leveraging the local update theorems proved in Section~\ref{ssec:localupdates}.

\begin{lemma}\label{lem:basecaseinvariants}
At initialization all of the invariants hold.
\end{lemma}
\begin{proof}
Since the weights and biases of the edges are all initialized to zero, all neurons are blank, proving the Blank/Active Invariant (Definition~\ref{def:blankactiveinvariant}). It also trivially follows that all active neurons compute an approximate monomial, proving the Approximate-Monomial Invariant (Definition~\ref{def:approximatemonomialinvariant}).

The function $f$ computed is identically-zero, since all the weights and biases are zero.
\end{proof}

\begin{lemma}\label{lem:inductivestepinvariants}
Each iteration of the inner loop maintains all of the invariants.
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}\label{lem:progressmade}
On each iteration of the outer loop, we learn a monomial with probability at least $1/(4N)$.
\end{lemma}
\begin{proof}
Since 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:cdguarantee}]
By Lemmas~\ref{lem:basecaseinvariants} and \ref{lem:inductivestepinvariants}, the invariants are maintained on each iteration at step~\ref{step:pickneuron}. Furthermore, each iteration of the outer loop has probability at least $1/(4N)$ to make progress and learn a monomial. Since the function we wish to learn is $s$-sparse in the Fourier basis, we can learn a new monomial at most $s$ times (since we never unlearn a monomial). Thus, after $\Tout = \Theta(s N \log(1/\delta))$ steps, we have learned all monomials with probability at least $1 - \delta$. Furthermore, by some invariant this means that each of these monomials is approximated to error at most $\epsilon_T$. This implies that the learned function is within $s \epsilon_T \leq \epsilon_{desired}$ of the true function, concluding the proof.
\end{proof}

\section{Technical lemmas}

\begin{align*}
\ell(a,b,c) &= \EE_x \frac{1}{2}((a x_1 + b x_2)^2 + c - x_1x_2)^2 \\
&= \frac{1}{2} ((2ab - 1)^2 + (a^2 + b^2 + c)^2)
\end{align*}

\begin{align*}
\frac{\partial \ell}{\partial a} = 2b(2ab - 1) + 2a(a^2 + b^2 + c)
\end{align*}
\begin{align*}
\frac{\partial \ell}{\partial c} = (a^2 + b^2 + c)
\end{align*}

\begin{align*}
\left(\frac{\partial \ell}{\partial a}\right)^2
\end{align*}
}









\begin{algorithm}\SetAlgoLined\DontPrintSemicolon
    \KwIn{
    Access to gradients of $\ellh$.
    }
    \KwOut{trained weights $A$, biases $b$ for the neural net}
    
    \BlankLine
    
    Initialize the biases $b_v = 0$ for all $v \in V \sm \Vin$, and the weights $A_e = 0$ for all $e \in E$.
    
    \While{$t = 1$ to $\Tout$}{
        \tcp{Pick a random neuron.}
        
        Pick $v \in V \in V \sm \Vin$ uniformly at random.
        \label{step:picksteepestneuron}
        
        \tcp{Perturb neuron weights slightly, to avoid saddle points}
        $w_v \gets w_v + z$, where $z$ is vector of independent entries drawn in $\mathrm{Unif}[-r,r]$.
        
        \tcp{Train the neuron to a stationary point of the empirical loss}
        \While{true}{
        Update $w_v \gets w_v - \eta \pd{\ellhr}{w_v}$  \label{step:traintostationary}
        
        If $\|\pd{\ellhr}{w_v}\| \leq \ein$, break.
         }
    \tcp{Round down small weights}
    $w_v \gets w_v \mbox{ rounded entrywise to 0}$ for each entry that is within a threshold $\tau$ from $0$
    }
    \caption{Block coordinate descent with early stopping, simpler version}
\label{alg:blockscdeasy}
\end{algorithm}




\begin{algorithm}\SetAlgoLined\DontPrintSemicolon
    \KwIn{
    Access to gradients of $\ellh$.
    }
    \KwOut{trained weights $A$, biases $b$ for the neural net}
    
    \BlankLine
    
    Initialize the biases $b_v = 0$ for all $v \in V \sm \Vin$, and the weights $A_e \sim \mathrm{Unif}[-r,r]$ for all $e \in E$.
    
    \While{true}{
        \tcp{Pick a random neuron among those with large gradient.}
        
        Pick $v \in V \sm \Vin$ uniformly at random among neurons such that $\|\pd{\ellhr}{w_v}\| > \epsilon_0$
        \label{step:picksteepestneuron}
        
        If there is no such neuron, break.
        
        \tcp{Train the neuron to a stationary point of the empirical loss}
        \While{true}{
        Update $w_v \gets w_v - \eta \pd{\ellhr}{w_v}$  \label{step:traintostationary}
        
        If $\|\pd{\ellhr}{w_v}\| \leq \ein$, break.
         }
    }
    \caption{Block coordinate descent with early stopping}
\label{alg:steepest}
\end{algorithm}
